Closed-loop Identification of a MSW Grate Incinerator using Bayesian Optimization for Selecting Model Inputs and Structure

The creation of low-order dynamic models for complex industrial systems is complicated by disturbances and limited sensor accuracy. This work presents a system identification procedure that uses machine learning methods and process knowledge to robustly identify a low-order closed-loop model of a municipal solid waste (MSW) grate incineration plant. These types of plants are known for their strong disturbances coming from fuel composition fluctuations. Using Bayesian optimization, the algorithm ranks and selects inputs from the available sensor data and chooses the model structure. This results in accurate models with low complexity while avoiding overfitting. The method is applied and validated using data of an industrial MSW incineration plant. The obtained models give excellent predictions and confidence intervals for the steam capacity and intermediate quantities such as supply air flow and flue gas temperature. The identified continuous-time models are fully given, and their step-response dynamics are discussed. The models can be used to develop model-based unit control schemes for grate incineration plants. The presented method shows great potential for the identification of over-actuated systems or disturbed systems with many sensors.

==> Figures/BasicModel_forprocessSketch.tex <==

\begin{axis}[%
width=6cm,
height=2cm,
at={(19.5cm,14.5cm)},
anchor=north east,
scale only axis,
xmin=0,
xmax=13.5,
ymin=0.5,
ymax=1.01,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xtick={\empty},
ytick={\empty}
]
\addplot [color=black, line width=1.2pt]
  table[row sep=crcr]{%
0	0.591023196609235\\
0.166666666666666	0.591023196609235\\
0.194444444444445	0.60148159901156\\
0.805555555555555	0.60148159901156\\
0.833333333333334	0.632946003680388\\
0.888888888888889	0.632946003680388\\
0.916666666666666	0.664410408349216\\
1.16666666666667	0.664410408349216\\
1.19444444444444	0.653952005946891\\
1.36111111111111	0.653952005946891\\
1.38888888888889	0.66305014705595\\
1.61111111111111	0.66305014705595\\
1.63888888888889	0.673508549458274\\
2	0.673508549458274\\
2.02777777777778	0.778337866501621\\
2.69444444444444	0.778337866501621\\
2.72222222222222	0.830719075975098\\
2.77777777777778	0.830719075975098\\
2.80555555555556	0.841467370128447\\
2.97222222222222	0.841467370128447\\
3	0.874916418323515\\
3.44444444444444	0.874916418323515\\
3.47222222222222	0.870434245865377\\
6.22222222222222	0.870434245865377\\
6.25	0.830295388031294\\
6.41666666666667	0.830295388031294\\
6.44444444444444	0.841467370128447\\
6.47222222222222	0.863744436226362\\
6.72222222222222	0.863744436226362\\
6.75	0.874202838628687\\
8.58333333333333	0.874202838628687\\
8.63888888888889	0.832280031557534\\
8.77777777777778	0.832280031557534\\
8.80555555555556	0.874202838628687\\
8.83333333333333	0.82182162915521\\
8.94444444444444	0.82182162915521\\
8.97222222222222	0.886110699786132\\
9.5	0.886110699786132\\
9.52777777777778	0.841467370128447\\
10.8333333333333	0.841467370128447\\
10.8611111111111	0.831031267091586\\
11.1944444444444	0.831031267091586\\
11.2222222222222	0.820461367861943\\
12.2222222222222	0.820461367861943\\
12.25	0.872931774797275\\
13.5	0.872931774797275\\
};

\addplot [color=red, line width=1.2pt]
  table[row sep=crcr]{%
1.00000000002876e-06	0.600001\\
1.99999999994649e-06	0.600001\\
};


\addplot[area legend, draw=none, fill=red, fill opacity=0.1]
table[row sep=crcr] {%
x	y\\
1e-06	0.600001\\
2e-06	0.600001\\
3e-06	0.600001\\
4e-06	0.600001\\
}--cycle;

\end{axis}

\begin{axis}[%
width=6cm,
height=2cm,
at={(19.5cm,12.25cm)},
anchor=north east,
scale only axis,
xmin=0,
xmax=13.5,
ymin=0.5,
ymax=1.01,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xtick={\empty},
ytick={\empty}
]
\addplot [color=black, line width=1.2pt, forget plot]
  table[row sep=crcr]{%
0	0.603400526198788\\
0.0555555555555554	0.599533730626804\\
0.111111111111111	0.592672255160597\\
0.138888888888889	0.592376885682089\\
0.166666666666666	0.594695688610027\\
0.194444444444445	0.593101576284054\\
0.222222222222221	0.595980626509208\\
0.25	0.596776599376703\\
0.277777777777779	0.591335724619761\\
0.305555555555555	0.59124691434454\\
0.333333333333334	0.582729739929961\\
0.361111111111111	0.585423632034457\\
0.388888888888889	0.592506893163659\\
0.416666666666666	0.595774161652255\\
0.444444444444445	0.596677545856823\\
0.472222222222221	0.594453841276067\\
0.5	0.594277683407496\\
0.527777777777779	0.59572845017837\\
0.555555555555555	0.597446313941125\\
0.638888888888889	0.595717636302068\\
0.666666666666666	0.595344364219509\\
0.694444444444445	0.599839445464523\\
0.722222222222221	0.600386755211922\\
0.75	0.594443171228326\\
0.777777777777779	0.590081330113263\\
0.805555555555555	0.587931830168861\\
0.833333333333334	0.587582062719813\\
0.861111111111111	0.597130250448538\\
0.888888888888889	0.602090596608789\\
0.916666666666666	0.601662200115427\\
0.944444444444445	0.595370771406017\\
0.972222222222221	0.598641048388686\\
1	0.599555619608646\\
1.02777777777778	0.608270204846878\\
1.05555555555556	0.607490986805578\\
1.08333333333333	0.611772337401517\\
1.11111111111111	0.611407614256013\\
1.13888888888889	0.613700965937193\\
1.16666666666667	0.615639771863346\\
1.19444444444444	0.617841334128387\\
1.22222222222222	0.617865352346648\\
1.25	0.616832841329668\\
1.27777777777778	0.623583808689997\\
1.30555555555556	0.628241435422453\\
1.33333333333333	0.635065880086687\\
1.36111111111111	0.636623290659484\\
1.38888888888889	0.647162659718513\\
1.41666666666667	0.652267460506442\\
1.44444444444444	0.660160936947056\\
1.47222222222222	0.664610575402339\\
1.5	0.667073150058799\\
1.52777777777778	0.665315973088145\\
1.55555555555556	0.667107141067181\\
1.61111111111111	0.667614279409284\\
1.63888888888889	0.667131357270746\\
1.66666666666667	0.663772661083733\\
1.69444444444444	0.663314349463951\\
1.72222222222222	0.659997276985768\\
1.75	0.659093537782352\\
1.77777777777778	0.663605795903123\\
1.80555555555556	0.660504113614007\\
1.83333333333333	0.659406362718846\\
1.86111111111111	0.662627191842256\\
1.88888888888889	0.657754608220344\\
1.91666666666667	0.658208683756465\\
1.94444444444444	0.654637051497449\\
1.97222222222222	0.654890364087006\\
2	0.649265174966143\\
2.02777777777778	0.648264124672854\\
2.05555555555556	0.651315220452672\\
2.08333333333333	0.649966481767144\\
2.11111111111111	0.650695122348331\\
2.16666666666667	0.646215340144728\\
2.19444444444444	0.654021739071144\\
2.22222222222222	0.655462575606553\\
2.25	0.668611927716505\\
2.27777777777778	0.671731115720787\\
2.30555555555556	0.673433722555734\\
2.33333333333333	0.676039300900872\\
2.36111111111111	0.679454789334546\\
2.38888888888889	0.678278564227668\\
2.41666666666667	0.678866452163884\\
2.44444444444444	0.686136498642204\\
2.47222222222222	0.692966492214305\\
2.5	0.695215504963118\\
2.52777777777778	0.697881838276839\\
2.55555555555556	0.697412193032863\\
2.58333333333333	0.709609257505171\\
2.61111111111111	0.720756792677975\\
2.63888888888889	0.727638541982213\\
2.66666666666667	0.723190825120053\\
2.69444444444444	0.716035150245354\\
2.72222222222222	0.713211489423276\\
2.75	0.715065683303965\\
2.77777777777778	0.719137478001192\\
2.80555555555556	0.726941301258609\\
2.83333333333333	0.732402530278671\\
2.86111111111111	0.744156031635365\\
2.88888888888889	0.743473104523531\\
2.91666666666667	0.745215697012412\\
2.94444444444444	0.744183397654423\\
2.97222222222222	0.742471062275735\\
3	0.747511300609109\\
3.02777777777778	0.753833664214557\\
3.05555555555556	0.755617078682191\\
3.08333333333333	0.754476965239903\\
3.11111111111111	0.757541065222778\\
3.13888888888889	0.763027488160908\\
3.16666666666667	0.772013068050896\\
3.19444444444444	0.77541000509094\\
3.22222222222222	0.779627913877711\\
3.25	0.783130229115352\\
3.27777777777778	0.788647434258159\\
3.30555555555556	0.796647466382481\\
3.33333333333333	0.806650245261936\\
3.36111111111111	0.824193305133017\\
3.38888888888889	0.831995436618559\\
3.41666666666667	0.841877014552034\\
3.44444444444444	0.847967509427958\\
3.47222222222222	0.849534009234286\\
3.5	0.869112949649255\\
3.52777777777778	0.893476574305398\\
3.55555555555556	0.897197767247265\\
3.58333333333333	0.913844989967204\\
3.61111111111111	0.917516816603458\\
3.63888888888889	0.914153224718905\\
3.66666666666667	0.922919372362488\\
3.69444444444444	0.916839125816182\\
3.72222222222222	0.909943302119135\\
3.75	0.90355487182665\\
3.77777777777778	0.892601778104535\\
3.80555555555556	0.886545196049491\\
3.83333333333333	0.884260222674207\\
3.86111111111111	0.880081931383893\\
3.88888888888889	0.875616727921336\\
3.91666666666667	0.869043886135159\\
3.94444444444444	0.871520249931612\\
3.97222222222222	0.864597034200912\\
4	0.85543244066789\\
4.05555555555556	0.841976995200975\\
4.08333333333333	0.840070781962741\\
4.11111111111111	0.849869771196321\\
4.13888888888889	0.850159163543927\\
4.16666666666667	0.848591779971526\\
4.19444444444444	0.845568668052298\\
4.22222222222222	0.846015973171058\\
4.25	0.848514437145274\\
4.27777777777778	0.853581476974492\\
4.30555555555556	0.856105974565233\\
4.33333333333333	0.864656971072108\\
4.36111111111111	0.868466386914612\\
4.38888888888889	0.871659883397401\\
4.41666666666667	0.868528755394919\\
4.44444444444444	0.862914149435758\\
4.47222222222222	0.861849716318234\\
4.5	0.863863195970623\\
4.52777777777778	0.862953884707379\\
4.58333333333333	0.854260627406951\\
4.61111111111111	0.854924725178121\\
4.63888888888889	0.860352075636301\\
4.66666666666667	0.857315452139229\\
4.69444444444444	0.848601978481959\\
4.72222222222222	0.84760868374017\\
4.75	0.850285147248385\\
4.77777777777778	0.84624639958515\\
4.80555555555556	0.844464177083248\\
4.86111111111111	0.840318895194731\\
4.88888888888889	0.843058767661613\\
4.94444444444444	0.853612653743157\\
4.97222222222222	0.852579769332099\\
5	0.851867252699\\
5.02777777777778	0.845692526307234\\
5.05555555555556	0.849870781871838\\
5.08333333333333	0.853077873478291\\
5.11111111111111	0.854795655951889\\
5.13888888888889	0.853926268183004\\
5.16666666666667	0.853647150501414\\
5.19444444444444	0.855926645226045\\
5.22222222222222	0.857436887929827\\
5.25	0.862643709415732\\
5.27777777777778	0.866159461470328\\
5.30555555555556	0.872981617990387\\
5.33333333333333	0.878343578300836\\
5.36111111111111	0.881733087257501\\
5.38888888888889	0.880475424441112\\
5.41666666666667	0.884416879088388\\
5.44444444444444	0.883717687709698\\
5.47222222222222	0.878737367844401\\
5.5	0.880814367041074\\
5.52777777777778	0.883679741462199\\
5.55555555555556	0.879271790717828\\
5.58333333333333	0.870977081207609\\
5.61111111111111	0.861203099113354\\
5.63888888888889	0.852411938164414\\
5.66666666666667	0.845241951426788\\
5.69444444444444	0.839610299947692\\
5.72222222222222	0.831791654706356\\
5.75	0.834358979317852\\
5.77777777777778	0.841545690545502\\
5.80555555555556	0.839361675456578\\
5.83333333333333	0.839498978478453\\
5.86111111111111	0.848747948020874\\
5.88888888888889	0.852762740000703\\
5.91666666666667	0.859862161428767\\
5.94444444444444	0.867528497246468\\
5.97222222222222	0.868447127865442\\
6	0.8656970289034\\
6.02777777777778	0.869968201497498\\
6.05555555555556	0.866470030442258\\
6.08333333333333	0.867325378668589\\
6.11111111111111	0.868438830708671\\
6.13888888888889	0.866236293580583\\
6.16666666666667	0.864915949690907\\
6.19444444444444	0.859979052873522\\
6.25	0.863982809732301\\
6.27777777777778	0.864863189507451\\
6.30555555555556	0.857255329719125\\
6.33333333333333	0.8533074862516\\
6.36111111111111	0.850924733889181\\
6.41666666666667	0.856328410880918\\
6.44444444444444	0.85423717645507\\
6.47222222222222	0.848928535101145\\
6.52777777777778	0.857489889078726\\
6.55555555555556	0.853731173367404\\
6.58333333333333	0.8517164374265\\
6.61111111111111	0.843789220276078\\
6.63888888888889	0.837269843283744\\
6.66666666666667	0.825303976174482\\
6.69444444444444	0.82706597488089\\
6.72222222222222	0.819471523338001\\
6.75	0.822816051639911\\
6.77777777777778	0.824336818926939\\
6.80555555555556	0.828331349430561\\
6.83333333333333	0.829219649957782\\
6.86111111111111	0.839409964616433\\
6.91666666666667	0.847880003863667\\
6.94444444444444	0.852743523590732\\
6.97222222222222	0.856691964809851\\
7	0.857205448354858\\
7.02777777777778	0.856372930776052\\
7.05555555555556	0.857297276733918\\
7.08333333333333	0.856266230607051\\
7.11111111111111	0.852355558967114\\
7.13888888888889	0.846081367844011\\
7.16666666666667	0.846725516957346\\
7.19444444444444	0.849140618457511\\
7.22222222222222	0.855941373160215\\
7.25	0.858438191538433\\
7.27777777777778	0.859115161896693\\
7.30555555555556	0.85431152101682\\
7.36111111111111	0.853175381436952\\
7.38888888888889	0.853597718514623\\
7.41666666666667	0.861596062649022\\
7.44444444444444	0.863315258980608\\
7.47222222222222	0.86883888340318\\
7.5	0.870639923808238\\
7.52777777777778	0.877787018675869\\
7.55555555555556	0.876824796920758\\
7.58333333333333	0.876691778231976\\
7.61111111111111	0.874618222047285\\
7.63888888888889	0.869678731621548\\
7.66666666666667	0.864340579789479\\
7.69444444444444	0.869967628169313\\
7.72222222222222	0.877728138981963\\
7.75	0.880728284749583\\
7.77777777777778	0.878462430062704\\
7.80555555555556	0.872088531941216\\
7.83333333333333	0.855920633978659\\
7.86111111111111	0.849153983980747\\
7.88888888888889	0.849665436161718\\
7.91666666666667	0.844937872787906\\
7.94444444444444	0.840708311042203\\
7.97222222222222	0.83838940276066\\
8	0.835427968131027\\
8.02777777777778	0.834944093789066\\
8.05555555555556	0.847558354600901\\
8.08333333333333	0.867538696497112\\
8.11111111111111	0.871468257201069\\
8.13888888888889	0.870988903353142\\
8.16666666666667	0.861677064214113\\
8.19444444444444	0.856719950132424\\
8.25	0.853738715515659\\
8.27777777777778	0.850808565304423\\
8.30555555555556	0.849986542718719\\
8.33333333333333	0.857858566300727\\
8.36111111111111	0.877968263963334\\
8.38888888888889	0.881418936795793\\
8.41666666666667	0.880255924972198\\
8.44444444444444	0.874283121053001\\
8.47222222222222	0.866220693908458\\
8.5	0.866772908140499\\
8.52777777777778	0.862695469501336\\
8.55555555555556	0.856083667651973\\
8.58333333333333	0.851529455964364\\
8.63888888888889	0.840354700250369\\
8.66666666666667	0.839652495626895\\
8.69444444444444	0.834332605900427\\
8.72222222222222	0.82512407909341\\
8.75	0.806360480891863\\
8.77777777777778	0.812037882390577\\
8.80555555555556	0.81366971702565\\
8.83333333333333	0.820669473898176\\
8.86111111111111	0.830079709979383\\
8.88888888888889	0.829416270536596\\
8.91666666666667	0.824969764088758\\
8.94444444444444	0.823831854401302\\
8.97222222222222	0.821783509612194\\
9	0.817980159336482\\
9.02777777777778	0.818923796063737\\
9.05555555555556	0.827992665448077\\
9.08333333333333	0.833563388044537\\
9.11111111111111	0.836616023277125\\
9.13888888888889	0.84789622620033\\
9.16666666666667	0.855212363839868\\
9.19444444444444	0.85726123081723\\
9.22222222222222	0.852681799069165\\
9.25	0.855832429617765\\
9.27777777777778	0.851535458098478\\
9.30555555555556	0.846276438202537\\
9.33333333333333	0.864956300881003\\
9.36111111111111	0.869719059811329\\
9.41666666666667	0.867729089061747\\
9.44444444444444	0.868476403919033\\
9.47222222222222	0.864396586203709\\
9.5	0.855185131746508\\
9.52777777777778	0.856511178816936\\
9.55555555555556	0.879710962240983\\
9.58333333333333	0.894529966855053\\
9.61111111111111	0.908572667792221\\
9.63888888888889	0.910769274222545\\
9.66666666666667	0.91151173046261\\
9.69444444444444	0.908861560673024\\
9.72222222222222	0.899842291784626\\
9.75	0.881099815305522\\
9.77777777777778	0.860369129575725\\
9.80555555555556	0.84162342376337\\
9.83333333333333	0.833692837264509\\
9.86111111111111	0.833183553575322\\
9.88888888888889	0.837014790640529\\
9.91666666666667	0.841654916993857\\
9.94444444444444	0.83912610800256\\
9.97222222222222	0.836843329305166\\
10	0.83337091318422\\
10.0277777777778	0.827657534774406\\
10.0555555555556	0.813417281055914\\
10.0833333333333	0.803422037392986\\
10.1111111111111	0.79570376427719\\
10.1388888888889	0.811864765195565\\
10.1666666666667	0.843431958026414\\
10.1944444444444	0.859548209199053\\
10.2222222222222	0.863695344724201\\
10.25	0.868124420748702\\
10.2777777777778	0.864571467574557\\
10.3055555555556	0.866512071810456\\
10.3333333333333	0.871656361961586\\
10.3611111111111	0.870365099505019\\
10.3888888888889	0.868694385648597\\
10.4166666666667	0.858709296237052\\
10.4444444444444	0.841558751856125\\
10.4722222222222	0.821317115779669\\
10.5	0.789969943681406\\
10.5277777777778	0.784663910674755\\
10.5555555555556	0.791654234817347\\
10.5833333333333	0.812177207835511\\
10.6111111111111	0.834118203989782\\
10.6388888888889	0.851251773641176\\
10.6666666666667	0.853491009931378\\
10.6944444444444	0.853503982228801\\
10.7222222222222	0.852565456415581\\
10.75	0.852638228183368\\
10.7777777777778	0.847918529263069\\
10.8055555555556	0.84872471942454\\
10.8333333333333	0.844607670565127\\
10.8611111111111	0.846528382017876\\
10.8888888888889	0.856326747428605\\
10.9166666666667	0.867598885135255\\
10.9444444444444	0.870759794659932\\
10.9722222222222	0.865910151011201\\
11	0.855073961956879\\
11.0277777777778	0.843721420444052\\
11.0555555555556	0.829257640180842\\
11.0833333333333	0.826011171440113\\
11.1111111111111	0.844585995470386\\
11.1388888888889	0.850827641483781\\
11.1666666666667	0.852665143951507\\
11.1944444444444	0.853070292545349\\
11.2222222222222	0.849844102383553\\
11.2777777777778	0.845029248180527\\
11.3055555555556	0.84362701277335\\
11.3333333333333	0.839379392757737\\
11.3611111111111	0.829028866352965\\
11.3888888888889	0.819172552131723\\
11.4166666666667	0.813572747290104\\
11.4444444444444	0.803743775570862\\
11.4722222222222	0.792645575958652\\
11.5	0.790949240154559\\
11.5277777777778	0.794126363145844\\
11.5555555555556	0.800021816898049\\
11.5833333333333	0.804483529109033\\
11.6111111111111	0.806601798321672\\
11.6388888888889	0.804883833592948\\
11.6666666666667	0.798776363299973\\
11.6944444444444	0.789039575442787\\
11.7222222222222	0.78133972618609\\
11.75	0.77569445854809\\
11.7777777777778	0.777658350676989\\
11.8055555555556	0.783292448453381\\
11.8333333333333	0.77419478736584\\
11.8611111111111	0.768588763260924\\
11.8888888888889	0.769546107744262\\
11.9166666666667	0.778419797760099\\
11.9444444444444	0.785025870242034\\
11.9722222222222	0.796953737430382\\
12	0.810743857959125\\
12.0277777777778	0.820672400442913\\
12.0555555555556	0.829650502509034\\
12.0833333333333	0.835309247678452\\
12.1111111111111	0.833124038721035\\
12.1388888888889	0.831459523618358\\
12.1666666666667	0.827432390246001\\
12.1944444444444	0.817395264646164\\
12.2222222222222	0.802472244815426\\
12.25	0.803259313856749\\
12.2777777777778	0.821259277329171\\
12.3055555555556	0.832368797381257\\
12.3333333333333	0.842743785979334\\
12.3611111111111	0.855726510574971\\
12.3888888888889	0.866957959580063\\
12.4166666666667	0.873186796039997\\
12.4444444444444	0.877115284653378\\
12.4722222222222	0.877639584948735\\
12.5	0.876247409910228\\
12.5277777777778	0.876992189635073\\
12.5555555555556	0.874002269922535\\
12.5833333333333	0.871891487799425\\
12.6111111111111	0.876785131292236\\
12.6388888888889	0.880307732981612\\
12.6666666666667	0.880085290195236\\
12.6944444444444	0.869166206697702\\
12.75	0.859158705172108\\
12.7777777777778	0.854475316880794\\
12.8055555555556	0.852847603580418\\
12.8333333333333	0.850310574992925\\
12.8611111111111	0.860311845262739\\
12.8888888888889	0.874181857348919\\
12.9166666666667	0.882645798057281\\
12.9444444444444	0.884822631974194\\
12.9722222222222	0.885944044486394\\
13	0.889126790813615\\
13.0555555555556	0.885575836506122\\
13.0833333333333	0.881508050771696\\
13.1111111111111	0.879401408087464\\
13.1388888888889	0.875066158687442\\
13.1666666666667	0.87103001250151\\
13.1944444444444	0.865946875621063\\
13.2222222222222	0.859881179201912\\
13.25	0.845428613490007\\
13.2777777777778	0.841057861962069\\
13.3055555555556	0.838897089013395\\
13.3333333333333	0.835901827249101\\
13.3611111111111	0.831584338010922\\
13.3888888888889	0.829183512092136\\
13.4166666666667	0.840068737177514\\
13.4444444444444	0.851272611882091\\
13.4722222222222	0.864371141957644\\
13.5	0.871040427647612\\
};
\addplot [color=red, line width=1.2pt, forget plot]
  table[row sep=crcr]{%
0	0.593516210715558\\
0.0277777777777786	0.591669459161329\\
0.0555555555555554	0.590334716966353\\
0.0833333333333339	0.588578847378137\\
0.111111111111111	0.587754351203671\\
0.138888888888889	0.585893240265502\\
0.166666666666666	0.586171143450141\\
0.194444444444445	0.585422749902643\\
0.222222222222221	0.587779828382706\\
0.25	0.586159731268356\\
0.277777777777779	0.586023326183803\\
0.305555555555555	0.584483834647427\\
0.333333333333334	0.584790525805751\\
0.361111111111111	0.584368939237709\\
0.388888888888889	0.586026166573562\\
0.416666666666666	0.585281132854421\\
0.472222222222221	0.581901171949697\\
0.5	0.580550621011843\\
0.527777777777779	0.582305046100288\\
0.555555555555555	0.582132575641991\\
0.583333333333334	0.581445516994362\\
0.611111111111111	0.579749756275403\\
0.638888888888889	0.579362580114898\\
0.666666666666666	0.577846185129365\\
0.694444444444445	0.579470058659664\\
0.722222222222221	0.579268939686896\\
0.75	0.578673094511016\\
0.833333333333334	0.584181049430288\\
0.861111111111111	0.589539470070319\\
0.888888888888889	0.593831334214325\\
0.916666666666666	0.595231832772518\\
0.944444444444445	0.597874646768895\\
0.972222222222221	0.60210482876618\\
1	0.604472544307963\\
1.02777777777778	0.609527448794333\\
1.05555555555556	0.611181256525194\\
1.08333333333333	0.612599047107967\\
1.11111111111111	0.615911341856894\\
1.13888888888889	0.617568298472902\\
1.16666666666667	0.619958838042724\\
1.22222222222222	0.621090048582557\\
1.25	0.622224244991143\\
1.27777777777778	0.625396925922576\\
1.30555555555556	0.626629253539209\\
1.33333333333333	0.627309048793672\\
1.36111111111111	0.626882989871573\\
1.38888888888889	0.630267941355916\\
1.44444444444444	0.633038362885239\\
1.5	0.634519122407145\\
1.52777777777778	0.634388603795067\\
1.55555555555556	0.635413412698854\\
1.58333333333333	0.636162275411273\\
1.61111111111111	0.636633366922723\\
1.66666666666667	0.636440505777431\\
1.69444444444444	0.636662420527273\\
1.72222222222222	0.638839482555627\\
1.75	0.64033898872256\\
1.77777777777778	0.642371454442319\\
1.83333333333333	0.64374060387615\\
1.86111111111111	0.64504692091039\\
1.88888888888889	0.644610944708026\\
1.91666666666667	0.644789315884889\\
1.94444444444444	0.647523669701821\\
1.97222222222222	0.64798971591741\\
2	0.64881588665258\\
2.02777777777778	0.651520670682485\\
2.05555555555556	0.658510911187046\\
2.08333333333333	0.664665288436955\\
2.11111111111111	0.669984557638402\\
2.13888888888889	0.673935007477212\\
2.16666666666667	0.679260340792551\\
2.22222222222222	0.691412594457278\\
2.25	0.698180270781252\\
2.27777777777778	0.703150728437382\\
2.30555555555556	0.706903974185263\\
2.36111111111111	0.715145247189223\\
2.38888888888889	0.718326070630862\\
2.41666666666667	0.721105055124486\\
2.47222222222222	0.73220971585256\\
2.52777777777778	0.737758254623191\\
2.55555555555556	0.739820808642657\\
2.58333333333333	0.744494706462637\\
2.61111111111111	0.7500619445468\\
2.63888888888889	0.752443817742186\\
2.66666666666667	0.753453031177473\\
2.69444444444444	0.751841774578045\\
2.72222222222222	0.752533039651539\\
2.75	0.757077002446552\\
2.77777777777778	0.760553270373505\\
2.80555555555556	0.767646111449158\\
2.83333333333333	0.772135960271397\\
2.86111111111111	0.777985375063984\\
2.91666666666667	0.784523723375699\\
2.97222222222222	0.788686233698403\\
3	0.793418240062699\\
3.02777777777778	0.800218729382003\\
3.05555555555556	0.805998792735181\\
3.08333333333333	0.809138154564891\\
3.11111111111111	0.815537528681579\\
3.13888888888889	0.818556738924428\\
3.16666666666667	0.827965767475481\\
3.19444444444444	0.833581761698998\\
3.22222222222222	0.836014382469333\\
3.25	0.840315419413749\\
3.27777777777778	0.845289438116605\\
3.30555555555556	0.850759194506878\\
3.33333333333333	0.852254621432353\\
3.36111111111111	0.858822557305514\\
3.38888888888889	0.861262099849936\\
3.44444444444444	0.864861354832632\\
3.47222222222222	0.86405026696883\\
3.5	0.870382033506704\\
3.52777777777778	0.877199393350054\\
3.55555555555556	0.873844627000302\\
3.58333333333333	0.874353770864172\\
3.61111111111111	0.876075220584479\\
3.63888888888889	0.873448012068183\\
3.66666666666667	0.878156249593774\\
3.69444444444444	0.876661016938712\\
3.72222222222222	0.871449933593752\\
3.75	0.871194764840787\\
3.77777777777778	0.86860805882961\\
3.80555555555556	0.867718693369495\\
3.83333333333333	0.869065872832369\\
3.86111111111111	0.872077308657754\\
3.88888888888889	0.872515663035189\\
3.91666666666667	0.871646563588246\\
3.94444444444444	0.877314693183521\\
3.97222222222222	0.876153547075159\\
4.05555555555556	0.876581541069529\\
4.08333333333333	0.875091261885419\\
4.11111111111111	0.87960500140338\\
4.13888888888889	0.879375139139801\\
4.16666666666667	0.876409906232885\\
4.19444444444444	0.875659398834905\\
4.22222222222222	0.874389086907923\\
4.25	0.874349233796087\\
4.27777777777778	0.873351768831206\\
4.30555555555556	0.875076236781744\\
4.33333333333333	0.875767875188705\\
4.36111111111111	0.877125440702292\\
4.38888888888889	0.876960766072104\\
4.41666666666667	0.875475414999576\\
4.44444444444444	0.874579125678464\\
4.47222222222222	0.876604363868731\\
4.5	0.877733679806736\\
4.52777777777778	0.877738236642591\\
4.55555555555556	0.875914854408613\\
4.58333333333333	0.874625117150936\\
4.61111111111111	0.874719890664002\\
4.63888888888889	0.87584095976492\\
4.66666666666667	0.873071072514666\\
4.69444444444444	0.872341533193181\\
4.72222222222222	0.874405451210826\\
4.75	0.877127156200693\\
4.77777777777778	0.877226820443976\\
4.80555555555556	0.879127084024764\\
4.83333333333333	0.880433812524306\\
4.88888888888889	0.884975320286488\\
4.91666666666667	0.885177442100778\\
4.94444444444444	0.88701920399868\\
4.97222222222222	0.886593161405946\\
5	0.88670229783404\\
5.02777777777778	0.883875220079611\\
5.05555555555556	0.889081964454926\\
5.08333333333333	0.888229309393271\\
5.11111111111111	0.888665737000828\\
5.13888888888889	0.888033472566365\\
5.16666666666667	0.888510933066945\\
5.19444444444444	0.890879862060634\\
5.22222222222222	0.891151425903265\\
5.25	0.889904965071162\\
5.27777777777778	0.889369462706364\\
5.30555555555556	0.890062346794334\\
5.33333333333333	0.891128761476653\\
5.36111111111111	0.890387936534719\\
5.38888888888889	0.8884382211466\\
5.41666666666667	0.888084286952649\\
5.44444444444444	0.886936530805418\\
5.47222222222222	0.884493565889301\\
5.5	0.886227812780065\\
5.52777777777778	0.888786488020353\\
5.55555555555556	0.887465197414986\\
5.58333333333333	0.885447582696351\\
5.61111111111111	0.884675479333856\\
5.63888888888889	0.884677556519589\\
5.66666666666667	0.885016003111884\\
5.69444444444444	0.88381486812191\\
5.72222222222222	0.882258635018664\\
5.75	0.883289134559666\\
5.77777777777778	0.885561846827667\\
5.80555555555556	0.881227052947066\\
5.83333333333333	0.881200431149315\\
5.86111111111111	0.882691149623849\\
5.88888888888889	0.881075821758809\\
5.91666666666667	0.879206721017102\\
5.94444444444444	0.880699753172687\\
5.97222222222222	0.876657656167144\\
6	0.874814499769458\\
6.02777777777778	0.877012569596703\\
6.05555555555556	0.877424387174655\\
6.08333333333333	0.876319569856721\\
6.11111111111111	0.877726216751981\\
6.13888888888889	0.878233875327373\\
6.16666666666667	0.877649663276971\\
6.19444444444444	0.876101642078499\\
6.22222222222222	0.877192646407023\\
6.25	0.875401851531846\\
6.27777777777778	0.872483734056313\\
6.30555555555556	0.866057780209147\\
6.33333333333333	0.863141990843138\\
6.36111111111111	0.859454148890126\\
6.38888888888889	0.858570825672427\\
6.41666666666667	0.855653262693293\\
6.44444444444444	0.851827751954046\\
6.47222222222222	0.850583877665905\\
6.5	0.850523540384758\\
6.52777777777778	0.854134639285878\\
6.55555555555556	0.853401886009065\\
6.58333333333333	0.85300929116312\\
6.61111111111111	0.85150667268309\\
6.63888888888889	0.850945478462139\\
6.66666666666667	0.849060743814253\\
6.69444444444444	0.852160395619832\\
6.72222222222222	0.851468019806624\\
6.75	0.853652151963168\\
6.77777777777778	0.854797573226151\\
6.80555555555556	0.856480814326789\\
6.83333333333333	0.856704417603805\\
6.86111111111111	0.861537202884934\\
6.88888888888889	0.86076131049453\\
6.91666666666667	0.861290966899501\\
6.94444444444444	0.86457373295141\\
7	0.868626932519904\\
7.02777777777778	0.868933991520636\\
7.05555555555556	0.871388357998033\\
7.08333333333333	0.870527334910028\\
7.11111111111111	0.87153152408538\\
7.13888888888889	0.870393559567901\\
7.16666666666667	0.872302287776277\\
7.19444444444444	0.874697231385827\\
7.22222222222222	0.87905214343885\\
7.25	0.878511397257901\\
7.27777777777778	0.878819284333604\\
7.30555555555556	0.878038586367346\\
7.33333333333333	0.879358594498383\\
7.36111111111111	0.882760283057991\\
7.38888888888889	0.884992567199847\\
7.41666666666667	0.886442478117814\\
7.44444444444444	0.885945719450991\\
7.47222222222222	0.887952503447389\\
7.5	0.887544575440391\\
7.52777777777778	0.889188558467012\\
7.55555555555556	0.887065536591527\\
7.58333333333333	0.886079474664745\\
7.61111111111111	0.885751549846313\\
7.63888888888889	0.883169364590405\\
7.66666666666667	0.879989855696831\\
7.69444444444444	0.884001296707485\\
7.72222222222222	0.885637145307497\\
7.75	0.884349200793606\\
7.77777777777778	0.881921755235386\\
7.80555555555556	0.878835521817384\\
7.83333333333333	0.875502773141354\\
7.86111111111111	0.876251221684583\\
7.88888888888889	0.87937362989592\\
7.91666666666667	0.877551901672131\\
7.94444444444444	0.877861737558291\\
7.97222222222222	0.87738730063303\\
8	0.876393467837655\\
8.02777777777778	0.875093423747163\\
8.05555555555556	0.878605647118336\\
8.08333333333333	0.883534602781301\\
8.13888888888889	0.878196393848835\\
8.16666666666667	0.87486796639233\\
8.19444444444444	0.87302490544173\\
8.22222222222222	0.873390776585525\\
8.25	0.871794219799876\\
8.27777777777778	0.870645011508246\\
8.30555555555556	0.87209459538839\\
8.33333333333333	0.874120822904844\\
8.36111111111111	0.883340743071077\\
8.38888888888889	0.881590457697186\\
8.41666666666667	0.879575398827361\\
8.44444444444444	0.877053295229899\\
8.47222222222222	0.87634390747113\\
8.5	0.878541957470334\\
8.55555555555556	0.876253295791969\\
8.58333333333333	0.876427375138974\\
8.61111111111111	0.875224706470938\\
8.63888888888889	0.87310764423143\\
8.66666666666667	0.8705132347114\\
8.69444444444444	0.868272480583869\\
8.72222222222222	0.86461716673195\\
8.75	0.854076805425299\\
8.80555555555556	0.854913435892204\\
8.83333333333333	0.85275025285172\\
8.86111111111111	0.853097782221953\\
8.88888888888889	0.848903283026985\\
8.91666666666667	0.843566657750136\\
8.94444444444444	0.84200743519922\\
8.97222222222222	0.839538956459007\\
9	0.841621742720216\\
9.05555555555556	0.852837056029633\\
9.08333333333333	0.856253654934664\\
9.13888888888889	0.864763255139987\\
9.16666666666667	0.869065167670232\\
9.19444444444444	0.87013062613322\\
9.22222222222222	0.867681887414369\\
9.25	0.872649889178495\\
9.27777777777778	0.87224929196837\\
9.30555555555556	0.874668463943216\\
9.33333333333333	0.886189112047356\\
9.36111111111111	0.888879831209735\\
9.38888888888889	0.889173860255116\\
9.41666666666667	0.888573130471412\\
9.44444444444444	0.889872535141397\\
9.5	0.886460355361985\\
9.52777777777778	0.887042992380493\\
9.55555555555556	0.891784893662368\\
9.58333333333333	0.8905181640823\\
9.63888888888889	0.885638257788244\\
9.66666666666667	0.884908733413894\\
9.69444444444444	0.883258446842383\\
9.72222222222222	0.879518207263036\\
9.75	0.874323983137327\\
9.77777777777778	0.871386856536525\\
9.80555555555556	0.870647039511226\\
9.86111111111111	0.87476998959615\\
9.88888888888889	0.875818170627793\\
9.91666666666667	0.87364652608283\\
9.94444444444444	0.873454784876763\\
9.97222222222222	0.872199826242088\\
10	0.869243900838796\\
10.0277777777778	0.866883569062839\\
10.0555555555556	0.863713531979885\\
10.0833333333333	0.861283134648115\\
10.1111111111111	0.861041265400111\\
10.1388888888889	0.865077755772624\\
10.1666666666667	0.873238363600935\\
10.1944444444444	0.872599078755695\\
10.2222222222222	0.870677417696616\\
10.25	0.869146166906784\\
10.2777777777778	0.867156576014937\\
10.3055555555556	0.86729570921236\\
10.3333333333333	0.866198210674776\\
10.3611111111111	0.862540232044019\\
10.3888888888889	0.860097325062007\\
10.4166666666667	0.857228632269406\\
10.4444444444444	0.855556065214646\\
10.4722222222222	0.855035459112216\\
10.5	0.851315353563381\\
10.5277777777778	0.854346430566114\\
10.5555555555556	0.8584326968532\\
10.6111111111111	0.866018437558674\\
10.6388888888889	0.867208747788121\\
10.6944444444444	0.861970011126894\\
10.7222222222222	0.859978983643499\\
10.75	0.859282043782844\\
10.7777777777778	0.857059110456669\\
10.8055555555556	0.857449487817586\\
10.8333333333333	0.855970618181267\\
10.8611111111111	0.856433178175195\\
10.8888888888889	0.859399772348823\\
10.9166666666667	0.858817686594591\\
10.9444444444444	0.855562710084969\\
10.9722222222222	0.851156855989148\\
11	0.845685721647374\\
11.0277777777778	0.842077283566011\\
11.0555555555556	0.841231428760775\\
11.0833333333333	0.841403287195996\\
11.1111111111111	0.84691849193314\\
11.1388888888889	0.847221376210582\\
11.1666666666667	0.845341085205119\\
11.1944444444444	0.843054632272842\\
11.2222222222222	0.840443223294393\\
11.25	0.838344853491273\\
11.2777777777778	0.836556604605697\\
11.3333333333333	0.83392783424782\\
11.3611111111111	0.830911012711534\\
11.3888888888889	0.828987993318862\\
11.4166666666667	0.827789280040065\\
11.4444444444444	0.82730285816028\\
11.4722222222222	0.826319762665564\\
11.5	0.827678306844968\\
11.5277777777778	0.829696098207487\\
11.5833333333333	0.830759637806619\\
11.6111111111111	0.8306441873087\\
11.6388888888889	0.829590241606397\\
11.6666666666667	0.826833527416548\\
11.6944444444444	0.826154319749493\\
11.7222222222222	0.824958404915424\\
11.75	0.824809734793821\\
11.7777777777778	0.827088603788447\\
11.8055555555556	0.82807045208409\\
11.8333333333333	0.826743258755439\\
11.8611111111111	0.828322474197693\\
11.9166666666667	0.833164169294903\\
11.9444444444444	0.83533028897388\\
12	0.838672147949151\\
12.0277777777778	0.839372484998908\\
12.0555555555556	0.838597981627926\\
12.0833333333333	0.83602037221346\\
12.1111111111111	0.835074722108914\\
12.1388888888889	0.832496554379254\\
12.1666666666667	0.830975418647064\\
12.1944444444444	0.828872016084269\\
12.2222222222222	0.826021945031137\\
12.25	0.831486138650057\\
12.2777777777778	0.840171229517836\\
12.3055555555556	0.845923610784865\\
12.3333333333333	0.8502684908928\\
12.3611111111111	0.853954427482867\\
12.3888888888889	0.85665605385031\\
12.4444444444444	0.858723699482583\\
12.5	0.860420848680251\\
12.5555555555556	0.860321613909331\\
12.5833333333333	0.861674489582636\\
12.6111111111111	0.864952006569393\\
12.6388888888889	0.866531332532437\\
12.6666666666667	0.866284323160821\\
12.6944444444444	0.864466346581711\\
12.7222222222222	0.865087722054277\\
12.75	0.865136026820156\\
12.7777777777778	0.867004271720077\\
12.8055555555556	0.870318952071308\\
12.8333333333333	0.873259585974765\\
12.8888888888889	0.884742418486418\\
12.9166666666667	0.887019901952332\\
12.9444444444444	0.886856083768013\\
12.9722222222222	0.887305314175832\\
13	0.888713241647315\\
13.0277777777778	0.887984665890762\\
13.0555555555556	0.887720975762265\\
13.0833333333333	0.887017481617006\\
13.1111111111111	0.88711942625863\\
13.1388888888889	0.885959252311578\\
13.1666666666667	0.888601176842286\\
13.1944444444444	0.888796450438525\\
13.2222222222222	0.888190545505063\\
13.25	0.884909992666074\\
13.2777777777778	0.885094172008994\\
13.3055555555556	0.884660945417247\\
13.3333333333333	0.884522018924388\\
13.3611111111111	0.882768266405099\\
13.3888888888889	0.882329909144831\\
13.4166666666667	0.883883209397711\\
13.4444444444444	0.884516060315859\\
13.4722222222222	0.883414956052093\\
13.5	0.882010805806043\\
};

\addplot[area legend, draw=none, fill=red, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
0	0.662226495207814\\
0.0277777777777778	0.660379743653584\\
0.0555555555555556	0.65904500145861\\
0.0833333333333333	0.657289131870394\\
0.111111111111111	0.656464635695926\\
0.138888888888889	0.654603524757757\\
0.166666666666667	0.654881427942397\\
0.194444444444444	0.654133034394899\\
0.222222222222222	0.656490112874962\\
0.25	0.654870015760612\\
0.277777777777778	0.654733610676058\\
0.305555555555556	0.653194119139683\\
0.333333333333333	0.653500810298006\\
0.361111111111111	0.653079223729964\\
0.388888888888889	0.654736451065818\\
0.416666666666667	0.653991417346677\\
0.444444444444444	0.652276168051882\\
0.472222222222222	0.650611456441953\\
0.5	0.6492609055041\\
0.527777777777778	0.651015330592544\\
0.555555555555556	0.650842860134246\\
0.583333333333333	0.650155801486618\\
0.611111111111111	0.648460040767658\\
0.638888888888889	0.648072864607153\\
0.666666666666667	0.646556469621621\\
0.694444444444444	0.64818034315192\\
0.722222222222222	0.647979224179151\\
0.75	0.647383379003272\\
0.777777777777778	0.649264938803799\\
0.805555555555556	0.650965124460168\\
0.833333333333333	0.652891333922543\\
0.861111111111111	0.658249754562574\\
0.888888888888889	0.662541618706581\\
0.916666666666667	0.663942117264774\\
0.944444444444444	0.666584931261151\\
0.972222222222222	0.670815113258435\\
1	0.673182828800219\\
1.02777777777778	0.678237733286589\\
1.05555555555556	0.679891541017449\\
1.08333333333333	0.681309331600222\\
1.11111111111111	0.68462162634915\\
1.13888888888889	0.686278582965157\\
1.16666666666667	0.68866912253498\\
1.19444444444444	0.689145152844358\\
1.22222222222222	0.689800333074812\\
1.25	0.6909345294834\\
1.27777777777778	0.694107210414833\\
1.30555555555556	0.695339538031464\\
1.33333333333333	0.696019333285928\\
1.36111111111111	0.695593274363828\\
1.38888888888889	0.698978225848171\\
1.41666666666667	0.700430871111617\\
1.44444444444444	0.701748647377495\\
1.47222222222222	0.70245037407298\\
1.5	0.7032294068994\\
1.52777777777778	0.703098888287322\\
1.55555555555556	0.704123697191109\\
1.58333333333333	0.704872559903528\\
1.61111111111111	0.705343651414978\\
1.63888888888889	0.705156211172881\\
1.66666666666667	0.705150790269686\\
1.69444444444444	0.705372705019528\\
1.72222222222222	0.707549767047883\\
1.75	0.709049273214816\\
1.77777777777778	0.711081738934575\\
1.80555555555556	0.711856900302532\\
1.83333333333333	0.712450888368406\\
1.86111111111111	0.713757205402646\\
1.88888888888889	0.713321229200282\\
1.91666666666667	0.713499600377146\\
1.94444444444444	0.716233954194076\\
1.97222222222222	0.716700000409665\\
2	0.717526171144835\\
2.02777777777778	0.720230955174741\\
2.05555555555556	0.727221195679302\\
2.08333333333333	0.733375572929212\\
2.11111111111111	0.738694842130658\\
2.13888888888889	0.742645291969468\\
2.16666666666667	0.747970625284806\\
2.19444444444444	0.754085645978566\\
2.22222222222222	0.760122878949533\\
2.25	0.766890555273509\\
2.27777777777778	0.771861012929638\\
2.30555555555556	0.775614258677518\\
2.33333333333333	0.779636189950417\\
2.36111111111111	0.783855531681479\\
2.38888888888889	0.787036355123118\\
2.41666666666667	0.789815339616741\\
2.44444444444444	0.795486268083498\\
2.47222222222222	0.800920000344816\\
2.5	0.803594659142182\\
2.52777777777778	0.806468539115447\\
2.55555555555556	0.808531093134912\\
2.58333333333333	0.813204990954894\\
2.61111111111111	0.818772229039056\\
2.63888888888889	0.821154102234443\\
2.66666666666667	0.822163315669729\\
2.69444444444444	0.820552059070301\\
2.72222222222222	0.821243324143795\\
2.75	0.825787286938808\\
2.77777777777778	0.82926355486576\\
2.80555555555556	0.836356395941415\\
2.83333333333333	0.840846244763652\\
2.86111111111111	0.84669565955624\\
2.88888888888889	0.849984626712359\\
2.91666666666667	0.853234007867955\\
2.94444444444444	0.855221234297421\\
2.97222222222222	0.857396518190659\\
3	0.862128524554954\\
3.02777777777778	0.868929013874258\\
3.05555555555556	0.874709077227437\\
3.08333333333333	0.877848439057148\\
3.11111111111111	0.884247813173835\\
3.13888888888889	0.887267023416683\\
3.16666666666667	0.896676051967736\\
3.19444444444444	0.902292046191254\\
3.22222222222222	0.904724666961589\\
3.25	0.909025703906005\\
3.27777777777778	0.913999722608861\\
3.30555555555556	0.919469478999134\\
3.33333333333333	0.920964905924609\\
3.36111111111111	0.92753284179777\\
3.38888888888889	0.929972384342193\\
3.41666666666667	0.931840009398404\\
3.44444444444444	0.933571639324888\\
3.47222222222222	0.932760551461086\\
3.5	0.939092317998959\\
3.52777777777778	0.945909677842311\\
3.55555555555556	0.942554911492558\\
3.58333333333333	0.943064055356427\\
3.61111111111111	0.944785505076735\\
3.63888888888889	0.942158296560439\\
3.66666666666667	0.94686653408603\\
3.69444444444444	0.945371301430968\\
3.72222222222222	0.940160218086008\\
3.75	0.939905049333042\\
3.77777777777778	0.937318343321866\\
3.80555555555556	0.93642897786175\\
3.83333333333333	0.937776157324625\\
3.86111111111111	0.94078759315001\\
3.88888888888889	0.941225947527444\\
3.91666666666667	0.940356848080502\\
3.94444444444444	0.946024977675777\\
3.97222222222222	0.944863831567414\\
4	0.944998164064832\\
4.02777777777778	0.94503441526083\\
4.05555555555556	0.945291825561784\\
4.08333333333333	0.943801546377676\\
4.11111111111111	0.948315285895636\\
4.13888888888889	0.948085423632057\\
4.16666666666667	0.94512019072514\\
4.19444444444444	0.944369683327162\\
4.22222222222222	0.943099371400179\\
4.25	0.943059518288342\\
4.27777777777778	0.942062053323461\\
4.30555555555556	0.943786521274001\\
4.33333333333333	0.94447815968096\\
4.36111111111111	0.945835725194547\\
4.38888888888889	0.945671050564361\\
4.41666666666667	0.944185699491831\\
4.44444444444444	0.94328941017072\\
4.47222222222222	0.945314648360987\\
4.5	0.946443964298992\\
4.52777777777778	0.946448521134847\\
4.55555555555556	0.944625138900868\\
4.58333333333333	0.943335401643192\\
4.61111111111111	0.943430175156258\\
4.63888888888889	0.944551244257176\\
4.66666666666667	0.941781357006922\\
4.69444444444444	0.941051817685436\\
4.72222222222222	0.943115735703083\\
4.75	0.945837440692949\\
4.77777777777778	0.945937104936231\\
4.80555555555556	0.947837368517021\\
4.83333333333333	0.949144097016561\\
4.86111111111111	0.951335095510461\\
4.88888888888889	0.953685604778743\\
4.91666666666667	0.953887726593034\\
4.94444444444444	0.955729488490936\\
4.97222222222222	0.955303445898202\\
5	0.955412582326295\\
5.02777777777778	0.952585504571867\\
5.05555555555556	0.957792248947181\\
5.08333333333333	0.956939593885526\\
5.11111111111111	0.957376021493083\\
5.13888888888889	0.956743757058621\\
5.16666666666667	0.9572212175592\\
5.19444444444444	0.95959014655289\\
5.22222222222222	0.95986171039552\\
5.25	0.958615249563417\\
5.27777777777778	0.958079747198619\\
5.30555555555556	0.95877263128659\\
5.33333333333333	0.959839045968909\\
5.36111111111111	0.959098221026974\\
5.38888888888889	0.957148505638857\\
5.41666666666667	0.956794571444905\\
5.44444444444444	0.955646815297673\\
5.47222222222222	0.953203850381556\\
5.5	0.954938097272321\\
5.52777777777778	0.957496772512608\\
5.55555555555556	0.956175481907242\\
5.58333333333333	0.954157867188607\\
5.61111111111111	0.953385763826111\\
5.63888888888889	0.953387841011845\\
5.66666666666667	0.95372628760414\\
5.69444444444444	0.952525152614166\\
5.72222222222222	0.950968919510919\\
5.75	0.951999419051922\\
5.77777777777778	0.954272131319923\\
5.80555555555556	0.949937337439322\\
5.83333333333333	0.94991071564157\\
5.86111111111111	0.951401434116105\\
5.88888888888889	0.949786106251065\\
5.91666666666667	0.947917005509357\\
5.94444444444444	0.949410037664943\\
5.97222222222222	0.945367940659399\\
6	0.943524784261713\\
6.02777777777778	0.945722854088958\\
6.05555555555556	0.94613467166691\\
6.08333333333333	0.945029854348976\\
6.11111111111111	0.946436501244237\\
6.13888888888889	0.946944159819629\\
6.16666666666667	0.946359947769227\\
6.19444444444444	0.944811926570755\\
6.22222222222222	0.945902930899279\\
6.25	0.944112136024101\\
6.27777777777778	0.941194018548568\\
6.30555555555556	0.934768064701403\\
6.33333333333333	0.931852275335393\\
6.36111111111111	0.928164433382382\\
6.38888888888889	0.927281110164683\\
6.41666666666667	0.924363547185549\\
6.44444444444444	0.920538036446302\\
6.47222222222222	0.91929416215816\\
6.5	0.919233824877014\\
6.52777777777778	0.922844923778134\\
6.55555555555556	0.922112170501321\\
6.58333333333333	0.921719575655375\\
6.61111111111111	0.920216957175345\\
6.63888888888889	0.919655762954395\\
6.66666666666667	0.917771028306508\\
6.69444444444444	0.920870680112087\\
6.72222222222222	0.92017830429888\\
6.75	0.922362436455423\\
6.77777777777778	0.923507857718407\\
6.80555555555556	0.925191098819043\\
6.83333333333333	0.925414702096061\\
6.86111111111111	0.930247487377189\\
6.88888888888889	0.929471594986785\\
6.91666666666667	0.930001251391756\\
6.94444444444444	0.933284017443666\\
6.97222222222222	0.935287442153852\\
7	0.937337217012159\\
7.02777777777778	0.937644276012892\\
7.05555555555556	0.940098642490288\\
7.08333333333333	0.939237619402283\\
7.11111111111111	0.940241808577637\\
7.13888888888889	0.939103844060158\\
7.16666666666667	0.941012572268532\\
7.19444444444444	0.943407515878082\\
7.22222222222222	0.947762427931106\\
7.25	0.947221681750156\\
7.27777777777778	0.94752956882586\\
7.30555555555556	0.946748870859602\\
7.33333333333333	0.948068878990639\\
7.36111111111111	0.951470567550246\\
7.38888888888889	0.953702851692103\\
7.41666666666667	0.95515276261007\\
7.44444444444444	0.954656003943247\\
7.47222222222222	0.956662787939644\\
7.5	0.956254859932646\\
7.52777777777778	0.957898842959267\\
7.55555555555556	0.955775821083781\\
7.58333333333333	0.954789759157001\\
7.61111111111111	0.954461834338568\\
7.63888888888889	0.95187964908266\\
7.66666666666667	0.948700140189086\\
7.69444444444444	0.952711581199741\\
7.72222222222222	0.954347429799752\\
7.75	0.953059485285862\\
7.77777777777778	0.950632039727641\\
7.80555555555556	0.947545806309641\\
7.83333333333333	0.944213057633611\\
7.86111111111111	0.944961506176839\\
7.88888888888889	0.948083914388175\\
7.91666666666667	0.946262186164387\\
7.94444444444444	0.946572022050547\\
7.97222222222222	0.946097585125286\\
8	0.945103752329911\\
8.02777777777778	0.94380370823942\\
8.05555555555556	0.947315931610592\\
8.08333333333333	0.952244887273558\\
8.11111111111111	0.949588252481486\\
8.13888888888889	0.94690667834109\\
8.16666666666667	0.943578250884585\\
8.19444444444444	0.941735189933986\\
8.22222222222222	0.942101061077781\\
8.25	0.940504504292131\\
8.27777777777778	0.939355296000502\\
8.30555555555556	0.940804879880646\\
8.33333333333333	0.942831107397099\\
8.36111111111111	0.952051027563332\\
8.38888888888889	0.950300742189442\\
8.41666666666667	0.948285683319617\\
8.44444444444444	0.945763579722155\\
8.47222222222222	0.945054191963385\\
8.5	0.94725224196259\\
8.52777777777778	0.946044941438737\\
8.55555555555556	0.944963580284224\\
8.58333333333333	0.945137659631229\\
8.61111111111111	0.943934990963194\\
8.63888888888889	0.941817928723686\\
8.66666666666667	0.939223519203655\\
8.69444444444444	0.936982765076125\\
8.72222222222222	0.933327451224205\\
8.75	0.922787089917555\\
8.77777777777778	0.923171719258078\\
8.80555555555556	0.92362372038446\\
8.83333333333333	0.921460537343975\\
8.86111111111111	0.921808066714208\\
8.88888888888889	0.917613567519241\\
8.91666666666667	0.912276942242391\\
8.94444444444444	0.910717719691476\\
8.97222222222222	0.908249240951262\\
9	0.910332027212472\\
9.02777777777778	0.915938006705865\\
9.05555555555556	0.921547340521888\\
9.08333333333333	0.92496393942692\\
9.11111111111111	0.929120937589636\\
9.13888888888889	0.933473539632243\\
9.16666666666667	0.937775452162487\\
9.19444444444444	0.938840910625475\\
9.22222222222222	0.936392171906625\\
9.25	0.941360173670751\\
9.27777777777778	0.940959576460624\\
9.30555555555556	0.943378748435472\\
9.33333333333333	0.954899396539611\\
9.36111111111111	0.957590115701991\\
9.38888888888889	0.957884144747372\\
9.41666666666667	0.957283414963669\\
9.44444444444444	0.958582819633653\\
9.47222222222222	0.956928966126953\\
9.5	0.955170639854241\\
9.52777777777778	0.955753276872749\\
9.55555555555556	0.960495178154623\\
9.58333333333333	0.959228448574556\\
9.61111111111111	0.956701133837165\\
9.63888888888889	0.9543485422805\\
9.66666666666667	0.95361901790615\\
9.69444444444444	0.951968731334638\\
9.72222222222222	0.948228491755293\\
9.75	0.943034267629583\\
9.77777777777778	0.94009714102878\\
9.80555555555556	0.939357324003482\\
9.83333333333333	0.94152614226868\\
9.86111111111111	0.943480274088405\\
9.88888888888889	0.944528455120049\\
9.91666666666667	0.942356810575085\\
9.94444444444444	0.942165069369019\\
9.97222222222222	0.940910110734343\\
10	0.937954185331052\\
10.0277777777778	0.935593853555094\\
10.0555555555556	0.93242381647214\\
10.0833333333333	0.929993419140371\\
10.1111111111111	0.929751549892366\\
10.1388888888889	0.93378804026488\\
10.1666666666667	0.94194864809319\\
10.1944444444444	0.94130936324795\\
10.2222222222222	0.939387702188871\\
10.25	0.93785645139904\\
10.2777777777778	0.935866860507192\\
10.3055555555556	0.936005993704616\\
10.3333333333333	0.934908495167032\\
10.3611111111111	0.931250516536275\\
10.3888888888889	0.928807609554263\\
10.4166666666667	0.925938916761661\\
10.4444444444444	0.924266349706901\\
10.4722222222222	0.923745743604472\\
10.5	0.920025638055637\\
10.5277777777778	0.92305671505837\\
10.5555555555556	0.927142981345456\\
10.5833333333333	0.930947994680412\\
10.6111111111111	0.93472872205093\\
10.6388888888889	0.935919032280377\\
10.6666666666667	0.933292339739632\\
10.6944444444444	0.930680295619149\\
10.7222222222222	0.928689268135755\\
10.75	0.9279923282751\\
10.7777777777778	0.925769394948925\\
10.8055555555556	0.926159772309841\\
10.8333333333333	0.924680902673523\\
10.8611111111111	0.92514346266745\\
10.8888888888889	0.928110056841078\\
10.9166666666667	0.927527971086847\\
10.9444444444444	0.924272994577225\\
10.9722222222222	0.919867140481404\\
11	0.91439600613963\\
11.0277777777778	0.910787568058267\\
11.0555555555556	0.909941713253031\\
11.0833333333333	0.910113571688252\\
11.1111111111111	0.915628776425395\\
11.1388888888889	0.915931660702838\\
11.1666666666667	0.914051369697374\\
11.1944444444444	0.911764916765098\\
11.2222222222222	0.909153507786649\\
11.25	0.907055137983529\\
11.2777777777778	0.905266889097952\\
11.3055555555556	0.904018204889017\\
11.3333333333333	0.902638118740076\\
11.3611111111111	0.89962129720379\\
11.3888888888889	0.897698277811118\\
11.4166666666667	0.89649956453232\\
11.4444444444444	0.896013142652536\\
11.4722222222222	0.895030047157819\\
11.5	0.896388591337223\\
11.5277777777778	0.898406382699742\\
11.5555555555556	0.898874870216412\\
11.5833333333333	0.899469922298875\\
11.6111111111111	0.899354471800956\\
11.6388888888889	0.898300526098652\\
11.6666666666667	0.895543811908804\\
11.6944444444444	0.89486460424175\\
11.7222222222222	0.89366868940768\\
11.75	0.893520019286076\\
11.7777777777778	0.895798888280703\\
11.8055555555556	0.896780736576346\\
11.8333333333333	0.895453543247695\\
11.8611111111111	0.897032758689948\\
11.8888888888889	0.899513850699332\\
11.9166666666667	0.901874453787159\\
11.9444444444444	0.904040573466136\\
11.9722222222222	0.905702082088703\\
12	0.907382432441406\\
12.0277777777778	0.908082769491164\\
12.0555555555556	0.907308266120182\\
12.0833333333333	0.904730656705715\\
12.1111111111111	0.903785006601169\\
12.1388888888889	0.90120683887151\\
12.1666666666667	0.89968570313932\\
12.1944444444444	0.897582300576524\\
12.2222222222222	0.894732229523392\\
12.25	0.900196423142312\\
12.2777777777778	0.908881514010091\\
12.3055555555556	0.91463389527712\\
12.3333333333333	0.918978775385055\\
12.3611111111111	0.922664711975123\\
12.3888888888889	0.925366338342566\\
12.4166666666667	0.926439289506299\\
12.4444444444444	0.927433983974838\\
12.4722222222222	0.928334915698764\\
12.5	0.929131133172506\\
12.5277777777778	0.929123314720127\\
12.5555555555556	0.929031898401587\\
12.5833333333333	0.930384774074893\\
12.6111111111111	0.933662291061649\\
12.6388888888889	0.935241617024694\\
12.6666666666667	0.934994607653077\\
12.6944444444444	0.933176631073968\\
12.7222222222222	0.933798006546532\\
12.75	0.933846311312413\\
12.7777777777778	0.935714556212333\\
12.8055555555556	0.939029236563564\\
12.8333333333333	0.941969870467021\\
12.8611111111111	0.947713065061909\\
12.8888888888889	0.953452702978674\\
12.9166666666667	0.955730186444588\\
12.9444444444444	0.955566368260269\\
12.9722222222222	0.956015598668087\\
13	0.95742352613957\\
13.0277777777778	0.956694950383018\\
13.0555555555556	0.95643126025452\\
13.0833333333333	0.955727766109262\\
13.1111111111111	0.955829710750886\\
13.1388888888889	0.954669536803834\\
13.1666666666667	0.957311461334542\\
13.1944444444444	0.957506734930781\\
13.2222222222222	0.956900829997319\\
13.25	0.95362027715833\\
13.2777777777778	0.95380445650125\\
13.3055555555556	0.953371229909502\\
13.3333333333333	0.953232303416643\\
13.3611111111111	0.951478550897356\\
13.3888888888889	0.951040193637087\\
13.4166666666667	0.952593493889967\\
13.4444444444444	0.953226344808115\\
13.4722222222222	0.952125240544348\\
13.5	0.950721090298299\\
13.5	0.813300521313787\\
13.4722222222222	0.814704671559837\\
13.4444444444444	0.815805775823603\\
13.4166666666667	0.815172924905455\\
13.3888888888889	0.813619624652576\\
13.3611111111111	0.814057981912844\\
13.3333333333333	0.815811734432131\\
13.3055555555556	0.815950660924991\\
13.2777777777778	0.816383887516739\\
13.25	0.816199708173818\\
13.2222222222222	0.819480261012807\\
13.1944444444444	0.820086165946269\\
13.1666666666667	0.819890892350031\\
13.1388888888889	0.817248967819322\\
13.1111111111111	0.818409141766374\\
13.0833333333333	0.81830719712475\\
13.0555555555556	0.819010691270009\\
13.0277777777778	0.819274381398506\\
13	0.820002957155058\\
12.9722222222222	0.818595029683575\\
12.9444444444444	0.818145799275758\\
12.9166666666667	0.818309617460076\\
12.8888888888889	0.816032133994163\\
12.8611111111111	0.810292496077397\\
12.8333333333333	0.804549301482509\\
12.8055555555556	0.801608667579052\\
12.7777777777778	0.798293987227822\\
12.75	0.796425742327901\\
12.7222222222222	0.796377437562021\\
12.6944444444444	0.795756062089456\\
12.6666666666667	0.797574038668566\\
12.6388888888889	0.797821048040182\\
12.6111111111111	0.796241722077137\\
12.5833333333333	0.792964205090381\\
12.5555555555556	0.791611329417075\\
12.5277777777778	0.791702745735615\\
12.5	0.791710564187995\\
12.4722222222222	0.790914346714253\\
12.4444444444444	0.790013414990327\\
12.4166666666667	0.789018720521787\\
12.3888888888889	0.787945769358054\\
12.3611111111111	0.785244142990611\\
12.3333333333333	0.781558206400544\\
12.3055555555556	0.777213326292609\\
12.2777777777778	0.771460945025579\\
12.25	0.762775854157801\\
12.2222222222222	0.757311660538881\\
12.1944444444444	0.760161731592012\\
12.1666666666667	0.762265134154808\\
12.1388888888889	0.763786269886998\\
12.1111111111111	0.766364437616658\\
12.0833333333333	0.767310087721204\\
12.0555555555556	0.769887697135671\\
12.0277777777778	0.770662200506652\\
12	0.769961863456895\\
11.9722222222222	0.768281513104191\\
11.9444444444444	0.766620004481624\\
11.9166666666667	0.764453884802648\\
11.8888888888889	0.76209328171482\\
11.8611111111111	0.759612189705437\\
11.8333333333333	0.758032974263184\\
11.8055555555556	0.759360167591835\\
11.7777777777778	0.758378319296191\\
11.75	0.756099450301565\\
11.7222222222222	0.756248120423168\\
11.6944444444444	0.757444035257238\\
11.6666666666667	0.758123242924293\\
11.6388888888889	0.76087995711414\\
11.6111111111111	0.761933902816444\\
11.5833333333333	0.762049353314363\\
11.5555555555556	0.761454301231901\\
11.5277777777778	0.760985813715231\\
11.5	0.758968022352712\\
11.4722222222222	0.757609478173308\\
11.4444444444444	0.758592573668024\\
11.4166666666667	0.759078995547809\\
11.3888888888889	0.760277708826606\\
11.3611111111111	0.762200728219279\\
11.3333333333333	0.765217549755564\\
11.3055555555556	0.766597635904505\\
11.2777777777778	0.76784632011344\\
11.25	0.769634568999017\\
11.2222222222222	0.771732938802138\\
11.1944444444444	0.774344347780586\\
11.1666666666667	0.776630800712862\\
11.1388888888889	0.778511091718327\\
11.1111111111111	0.778208207440884\\
11.0833333333333	0.772693002703741\\
11.0555555555556	0.772521144268519\\
11.0277777777778	0.773366999073755\\
11	0.776975437155119\\
10.9722222222222	0.782446571496892\\
10.9444444444444	0.786852425592713\\
10.9166666666667	0.790107402102335\\
10.8888888888889	0.790689487856567\\
10.8611111111111	0.787722893682939\\
10.8333333333333	0.787260333689012\\
10.8055555555556	0.78873920332533\\
10.7777777777778	0.788348825964413\\
10.75	0.790571759290589\\
10.7222222222222	0.791268699151244\\
10.6944444444444	0.793259726634638\\
10.6666666666667	0.79587177075512\\
10.6388888888889	0.798498463295865\\
10.6111111111111	0.797308153066419\\
10.5833333333333	0.7935274256959\\
10.5555555555556	0.789722412360944\\
10.5277777777778	0.785636146073858\\
10.5	0.782605069071125\\
10.4722222222222	0.786325174619961\\
10.4444444444444	0.78684578072239\\
10.4166666666667	0.78851834777715\\
10.3888888888889	0.791387040569751\\
10.3611111111111	0.793829947551763\\
10.3333333333333	0.797487926182521\\
10.3055555555556	0.798585424720105\\
10.2777777777778	0.798446291522681\\
10.25	0.800435882414528\\
10.2222222222222	0.801967133204359\\
10.1944444444444	0.803888794263439\\
10.1666666666667	0.804528079108679\\
10.1388888888889	0.796367471280368\\
10.1111111111111	0.792330980907854\\
10.0833333333333	0.79257285015586\\
10.0555555555556	0.795003247487629\\
10.0277777777778	0.798173284570583\\
10	0.80053361634654\\
9.97222222222222	0.803489541749832\\
9.94444444444444	0.804744500384507\\
9.91666666666667	0.804936241590574\\
9.88888888888889	0.807107886135537\\
9.86111111111111	0.806059705103893\\
9.83333333333333	0.804105573284168\\
9.80555555555556	0.80193675501897\\
9.77777777777778	0.802676572044268\\
9.75	0.805613698645071\\
9.72222222222222	0.810807922770781\\
9.69444444444444	0.814548162350127\\
9.66666666666667	0.816198448921638\\
9.63888888888889	0.816927973295988\\
9.61111111111111	0.819280564852653\\
9.58333333333333	0.821807879590044\\
9.55555555555556	0.823074609170112\\
9.52777777777778	0.818332707888238\\
9.5	0.81775007086973\\
9.47222222222222	0.819508397142442\\
9.44444444444444	0.821162250649141\\
9.41666666666667	0.819862845979157\\
9.38888888888889	0.82046357576286\\
9.36111111111111	0.82016954671748\\
9.33333333333333	0.8174788275551\\
9.30555555555556	0.805958179450961\\
9.27777777777778	0.803539007476113\\
9.25	0.803939604686239\\
9.22222222222222	0.798971602922113\\
9.19444444444444	0.801420341640963\\
9.16666666666667	0.800354883177976\\
9.13888888888889	0.796052970647731\\
9.11111111111111	0.791700368605124\\
9.08333333333333	0.787543370442408\\
9.05555555555556	0.784126771537377\\
9.02777777777778	0.778517437721353\\
9	0.772911458227961\\
8.97222222222222	0.770828671966751\\
8.94444444444444	0.773297150706964\\
8.91666666666667	0.77485637325788\\
8.88888888888889	0.780192998534729\\
8.86111111111111	0.784387497729697\\
8.83333333333333	0.784039968359464\\
8.80555555555556	0.786203151399949\\
8.77777777777778	0.785751150273567\\
8.75	0.785366520933043\\
8.72222222222222	0.795906882239693\\
8.69444444444444	0.799562196091613\\
8.66666666666667	0.801802950219143\\
8.63888888888889	0.804397359739174\\
8.61111111111111	0.806514421978683\\
8.58333333333333	0.807717090646718\\
8.55555555555556	0.807543011299713\\
8.52777777777778	0.808624372454225\\
8.5	0.809831672978078\\
8.47222222222222	0.807633622978873\\
8.44444444444444	0.808343010737644\\
8.41666666666667	0.810865114335105\\
8.38888888888889	0.812880173204931\\
8.36111111111111	0.814630458578821\\
8.33333333333333	0.805410538412588\\
8.30555555555556	0.803384310896135\\
8.27777777777778	0.80193472701599\\
8.25	0.803083935307619\\
8.22222222222222	0.804680492093269\\
8.19444444444444	0.804314620949475\\
8.16666666666667	0.806157681900074\\
8.13888888888889	0.809486109356579\\
8.11111111111111	0.812167683496975\\
8.08333333333333	0.814824318289046\\
8.05555555555556	0.809895362626081\\
8.02777777777778	0.806383139254908\\
8	0.807683183345399\\
7.97222222222222	0.808677016140774\\
7.94444444444444	0.809151453066036\\
7.91666666666667	0.808841617179876\\
7.88888888888889	0.810663345403663\\
7.86111111111111	0.807540937192328\\
7.83333333333333	0.806792488649099\\
7.80555555555556	0.810125237325129\\
7.77777777777778	0.813211470743129\\
7.75	0.815638916301351\\
7.72222222222222	0.81692686081524\\
7.69444444444444	0.815291012215229\\
7.66666666666667	0.811279571204574\\
7.63888888888889	0.814459080098148\\
7.61111111111111	0.817041265354057\\
7.58333333333333	0.817369190172489\\
7.55555555555556	0.81835525209927\\
7.52777777777778	0.820478273974756\\
7.5	0.818834290948135\\
7.47222222222222	0.819242218955133\\
7.44444444444444	0.817235434958735\\
7.41666666666667	0.817732193625559\\
7.38888888888889	0.816282282707591\\
7.36111111111111	0.814049998565734\\
7.33333333333333	0.810648310006127\\
7.30555555555556	0.80932830187509\\
7.27777777777778	0.810108999841348\\
7.25	0.809801112765644\\
7.22222222222222	0.810341858946594\\
7.19444444444444	0.805986946893571\\
7.16666666666667	0.803592003284021\\
7.13888888888889	0.801683275075646\\
7.11111111111111	0.802821239593125\\
7.08333333333333	0.801817050417772\\
7.05555555555556	0.802678073505776\\
7.02777777777778	0.800223707028381\\
7	0.799916648027648\\
6.97222222222222	0.797866873169341\\
6.94444444444444	0.795863448459154\\
6.91666666666667	0.792580682407245\\
6.88888888888889	0.792051026002274\\
6.86111111111111	0.792826918392678\\
6.83333333333333	0.787994133111549\\
6.80555555555556	0.787770529834532\\
6.77777777777778	0.786087288733896\\
6.75	0.784941867470912\\
6.72222222222222	0.782757735314369\\
6.69444444444444	0.783450111127576\\
6.66666666666667	0.780350459321997\\
6.63888888888889	0.782235193969884\\
6.61111111111111	0.782796388190834\\
6.58333333333333	0.784299006670864\\
6.55555555555556	0.784691601516809\\
6.52777777777778	0.785424354793623\\
6.5	0.781813255892502\\
6.47222222222222	0.781873593173648\\
6.44444444444444	0.78311746746179\\
6.41666666666667	0.786942978201037\\
6.38888888888889	0.789860541180171\\
6.36111111111111	0.79074386439787\\
6.33333333333333	0.794431706350881\\
6.30555555555556	0.797347495716891\\
6.27777777777778	0.803773449564057\\
6.25	0.806691567039589\\
6.22222222222222	0.808482361914767\\
6.19444444444444	0.807391357586243\\
6.16666666666667	0.808939378784716\\
6.13888888888889	0.809523590835118\\
6.11111111111111	0.809015932259726\\
6.08333333333333	0.807609285364465\\
6.05555555555556	0.808714102682398\\
6.02777777777778	0.808302285104447\\
6	0.806104215277202\\
5.97222222222222	0.807947371674887\\
5.94444444444444	0.811989468680431\\
5.91666666666667	0.810496436524845\\
5.88888888888889	0.812365537266554\\
5.86111111111111	0.813980865131594\\
5.83333333333333	0.812490146657058\\
5.80555555555556	0.81251676845481\\
5.77777777777778	0.816851562335412\\
5.75	0.81457885006741\\
5.72222222222222	0.813548350526408\\
5.69444444444444	0.815104583629654\\
5.66666666666667	0.816305718619629\\
5.63888888888889	0.815967272027334\\
5.61111111111111	0.815965194841599\\
5.58333333333333	0.816737298204095\\
5.55555555555556	0.81875491292273\\
5.52777777777778	0.820076203528097\\
5.5	0.81751752828781\\
5.47222222222222	0.815783281397044\\
5.44444444444444	0.818226246313161\\
5.41666666666667	0.819374002460393\\
5.38888888888889	0.819727936654345\\
5.36111111111111	0.821677652042462\\
5.33333333333333	0.822418476984397\\
5.30555555555556	0.821352062302078\\
5.27777777777778	0.820659178214108\\
5.25	0.821194680578906\\
5.22222222222222	0.822441141411009\\
5.19444444444444	0.822169577568378\\
5.16666666666667	0.819800648574689\\
5.13888888888889	0.819323188074109\\
5.11111111111111	0.819955452508571\\
5.08333333333333	0.819519024901015\\
5.05555555555556	0.82037167996267\\
5.02777777777778	0.815164935587356\\
5	0.817992013341783\\
4.97222222222222	0.81788287691369\\
4.94444444444444	0.818308919506424\\
4.91666666666667	0.816467157608523\\
4.88888888888889	0.816265035794232\\
4.86111111111111	0.813914526525949\\
4.83333333333333	0.81172352803205\\
4.80555555555556	0.810416799532509\\
4.77777777777778	0.80851653595172\\
4.75	0.808416871708438\\
4.72222222222222	0.805695166718571\\
4.69444444444444	0.803631248700924\\
4.66666666666667	0.80436078802241\\
4.63888888888889	0.807130675272664\\
4.61111111111111	0.806009606171746\\
4.58333333333333	0.80591483265868\\
4.55555555555556	0.807204569916356\\
4.52777777777778	0.809027952150335\\
4.5	0.809023395314481\\
4.47222222222222	0.807894079376475\\
4.44444444444444	0.805868841186209\\
4.41666666666667	0.80676513050732\\
4.38888888888889	0.808250481579849\\
4.36111111111111	0.808415156210035\\
4.33333333333333	0.807057590696449\\
4.30555555555556	0.806365952289489\\
4.27777777777778	0.80464148433895\\
4.25	0.805638949303831\\
4.22222222222222	0.805678802415667\\
4.19444444444444	0.80694911434265\\
4.16666666666667	0.807699621740628\\
4.13888888888889	0.810664854647546\\
4.11111111111111	0.810894716911124\\
4.08333333333333	0.806380977393164\\
4.05555555555556	0.807871256577273\\
4.02777777777778	0.807613846276318\\
4	0.80757759508032\\
3.97222222222222	0.807443262582903\\
3.94444444444444	0.808604408691265\\
3.91666666666667	0.802936279095991\\
3.88888888888889	0.803805378542933\\
3.86111111111111	0.803367024165499\\
3.83333333333333	0.800355588340114\\
3.80555555555556	0.799008408877239\\
3.77777777777778	0.799897774337355\\
3.75	0.802484480348531\\
3.72222222222222	0.802739649101497\\
3.69444444444444	0.807950732446457\\
3.66666666666667	0.809445965101518\\
3.63888888888889	0.804737727575928\\
3.61111111111111	0.807364936092224\\
3.58333333333333	0.805643486371916\\
3.55555555555556	0.805134342508046\\
3.52777777777778	0.808489108857799\\
3.5	0.801671749014448\\
3.47222222222222	0.795339982476575\\
3.44444444444444	0.796151070340376\\
3.41666666666667	0.794419440413892\\
3.38888888888889	0.792551815357681\\
3.36111111111111	0.790112272813259\\
3.33333333333333	0.783544336940098\\
3.30555555555556	0.782048910014623\\
3.27777777777778	0.77657915362435\\
3.25	0.771605134921493\\
3.22222222222222	0.767304097977078\\
3.19444444444444	0.764871477206742\\
3.16666666666667	0.759255482983225\\
3.13888888888889	0.749846454432172\\
3.11111111111111	0.746827244189323\\
3.08333333333333	0.740427870072636\\
3.05555555555556	0.737288508242926\\
3.02777777777778	0.731508444889747\\
3	0.724707955570443\\
2.97222222222222	0.719975949206148\\
2.94444444444444	0.71780066531291\\
2.91666666666667	0.715813438883444\\
2.88888888888889	0.712564057727847\\
2.86111111111111	0.709275090571728\\
2.83333333333333	0.703425675779141\\
2.80555555555556	0.698935826956903\\
2.77777777777778	0.691842985881249\\
2.75	0.688366717954296\\
2.72222222222222	0.683822755159283\\
2.69444444444444	0.683131490085789\\
2.66666666666667	0.684742746685218\\
2.63888888888889	0.683733533249931\\
2.61111111111111	0.681351660054545\\
2.58333333333333	0.675784421970382\\
2.55555555555556	0.671110524150401\\
2.52777777777778	0.669047970130936\\
2.5	0.666174090157671\\
2.47222222222222	0.663499431360304\\
2.44444444444444	0.658065699098986\\
2.41666666666667	0.65239477063223\\
2.38888888888889	0.649615786138606\\
2.36111111111111	0.646434962696968\\
2.33333333333333	0.642215620965905\\
2.30555555555556	0.638193689693006\\
2.27777777777778	0.634440443945127\\
2.25	0.629469986288997\\
2.22222222222222	0.622702309965022\\
2.19444444444444	0.616665076994055\\
2.16666666666667	0.610550056300294\\
2.13888888888889	0.605224722984956\\
2.11111111111111	0.601274273146147\\
2.08333333333333	0.5959550039447\\
2.05555555555556	0.58980062669479\\
2.02777777777778	0.58281038619023\\
2	0.580105602160324\\
1.97222222222222	0.579279431425153\\
1.94444444444444	0.578813385209564\\
1.91666666666667	0.576079031392634\\
1.88888888888889	0.57590066021577\\
1.86111111111111	0.576336636418134\\
1.83333333333333	0.575030319383894\\
1.80555555555556	0.574436331318021\\
1.77777777777778	0.573661169950063\\
1.75	0.571628704230304\\
1.72222222222222	0.570129198063371\\
1.69444444444444	0.567952136035017\\
1.66666666666667	0.567730221285174\\
1.63888888888889	0.567735642188369\\
1.61111111111111	0.567923082430466\\
1.58333333333333	0.567451990919017\\
1.55555555555556	0.566703128206598\\
1.52777777777778	0.56567831930281\\
1.5	0.565808837914889\\
1.47222222222222	0.565029805088468\\
1.44444444444444	0.564328078392984\\
1.41666666666667	0.563010302127105\\
1.38888888888889	0.56155765686366\\
1.36111111111111	0.558172705379317\\
1.33333333333333	0.558598764301417\\
1.30555555555556	0.557918969046952\\
1.27777777777778	0.556686641430321\\
1.25	0.553513960498888\\
1.22222222222222	0.552379764090301\\
1.19444444444444	0.551724583859847\\
1.16666666666667	0.551248553550469\\
1.13888888888889	0.548858013980646\\
1.11111111111111	0.547201057364638\\
1.08333333333333	0.54388876261571\\
1.05555555555556	0.542470972032938\\
1.02777777777778	0.540817164302077\\
1	0.535762259815707\\
0.972222222222222	0.533394544273923\\
0.944444444444444	0.529164362276639\\
0.916666666666667	0.526521548280263\\
0.888888888888889	0.52512104972207\\
0.861111111111111	0.520829185578063\\
0.833333333333333	0.515470764938032\\
0.805555555555556	0.513544555475657\\
0.777777777777778	0.511844369819287\\
0.75	0.509962810018761\\
0.722222222222222	0.51055865519464\\
0.694444444444444	0.510759774167409\\
0.666666666666667	0.50913590063711\\
0.638888888888889	0.510652295622641\\
0.611111111111111	0.511039471783146\\
0.583333333333333	0.512735232502107\\
0.555555555555556	0.513422291149735\\
0.527777777777778	0.513594761608032\\
0.5	0.511840336519588\\
0.472222222222222	0.513190887457441\\
0.444444444444444	0.514855599067371\\
0.416666666666667	0.516570848362166\\
0.388888888888889	0.517315882081307\\
0.361111111111111	0.515658654745453\\
0.333333333333333	0.516080241313495\\
0.305555555555556	0.515773550155171\\
0.277777777777778	0.517313041691546\\
0.25	0.5174494467761\\
0.222222222222222	0.51906954389045\\
0.194444444444444	0.516712465410387\\
0.166666666666667	0.517460858957885\\
0.138888888888889	0.517182955773246\\
0.111111111111111	0.519044066711415\\
0.0833333333333333	0.519868562885882\\
0.0555555555555556	0.521624432474098\\
0.0277777777777778	0.522959174669073\\
0	0.524805926223302\\
}--cycle;
\end{axis}

==> Figures/GP_n2_v1.tex <==
\begin{axis}[%
width=5.5cm,
height=3cm,
at={(39.75cm,15.75cm)},
anchor = north east,
scale only axis,
xmin=0,
xmax=6,
xtick={\empty},
ymin=-1,
ymax=0,
ytick={\empty},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]
\addplot [color=blue, line width=1.2pt, forget plot]
  table[row sep=crcr]{%
0	-0.634078614219124\\
0.12012012012012	-0.635969289685819\\
0.21021021021021	-0.6384194897729\\
0.282282282282282	-0.641374340169751\\
0.348348348348348	-0.645179549902262\\
0.402402402402402	-0.649319916814719\\
0.45045045045045	-0.653972781388276\\
0.498498498498498	-0.659730204559189\\
0.54054054054054	-0.665829613793346\\
0.582582582582583	-0.673064097135586\\
0.618618618618619	-0.680270751559875\\
0.654654654654655	-0.688487114215132\\
0.69069069069069	-0.697774856610486\\
0.726726726726727	-0.70817100090571\\
0.762762762762763	-0.719675742717579\\
0.798798798798799	-0.732237462483051\\
0.840840840840841	-0.748062236574688\\
0.894894894894895	-0.769688347088265\\
0.966966966966967	-0.798565794580966\\
0.996996996996997	-0.809597056233689\\
1.02102102102102	-0.81754836015032\\
1.04504504504505	-0.824438780568435\\
1.06906906906907	-0.829997522641141\\
1.08708708708709	-0.833135237734115\\
1.10510510510511	-0.835279893242776\\
1.12312312312312	-0.836355312026121\\
1.14114114114114	-0.836317947752766\\
1.15915915915916	-0.835169411495376\\
1.17717717717718	-0.832955850579362\\
1.1951951951952	-0.829755168196851\\
1.21321321321321	-0.82566548554616\\
1.23723723723724	-0.819019733349351\\
1.26126126126126	-0.811259058326114\\
1.29129129129129	-0.800394186678132\\
1.33333333333333	-0.783856007683283\\
1.43543543543544	-0.742968937568349\\
1.47747747747748	-0.727514395432599\\
1.51351351351351	-0.715330263854134\\
1.54954954954955	-0.704229117230366\\
1.58558558558559	-0.694241653865023\\
1.62162162162162	-0.685352583844733\\
1.65765765765766	-0.677514574963936\\
1.69369369369369	-0.670659442062886\\
1.73573573573574	-0.663796485153359\\
1.77777777777778	-0.65802521619996\\
1.82582582582583	-0.652590640237938\\
1.87387387387387	-0.648208604969273\\
1.92792792792793	-0.644317352221545\\
1.98798798798799	-0.641027351401368\\
2.06006006006006	-0.638176757590395\\
2.14414414414414	-0.635940137659303\\
2.25225225225225	-0.634196079429098\\
2.3963963963964	-0.63300443475931\\
2.63663663663664	-0.632246022825226\\
3.10510510510511	-0.630889619569306\\
3.24924924924925	-0.629343856624516\\
3.35135135135135	-0.627255723503221\\
3.43543543543544	-0.624479251269753\\
3.5015015015015	-0.621307141573416\\
3.56156156156156	-0.617391666602488\\
3.61561561561562	-0.612787358682727\\
3.66366366366366	-0.607632993895247\\
3.70570570570571	-0.602147713961879\\
3.74774774774775	-0.595610118576898\\
3.78978978978979	-0.587882664168926\\
3.82582582582583	-0.580212934495957\\
3.86186186186186	-0.571502280647918\\
3.8978978978979	-0.561699205785576\\
3.93393393393393	-0.550782212718772\\
3.96996996996997	-0.538773280658165\\
4.01201201201201	-0.523496039636028\\
4.06006006006006	-0.504709074839767\\
4.17417417417417	-0.459316905497871\\
4.2042042042042	-0.448923586888487\\
4.22822822822823	-0.441687627401842\\
4.25225225225225	-0.435702544096179\\
4.27027027027027	-0.432195150413885\\
4.28828828828829	-0.429644062592615\\
4.30630630630631	-0.42813503008474\\
4.32432432432432	-0.42772620948374\\
4.34234234234234	-0.428435054741573\\
4.36036036036036	-0.430231876492567\\
4.37837837837838	-0.433049878896198\\
4.3963963963964	-0.436797803510048\\
4.42042042042042	-0.44305744375347\\
4.44444444444444	-0.450513128882705\\
4.47447447447447	-0.46110612059565\\
4.51051051051051	-0.475041698153913\\
4.64864864864865	-0.529775982600455\\
4.68468468468468	-0.54250356619741\\
4.72072072072072	-0.554188956653443\\
4.75675675675676	-0.564770286242628\\
4.79279279279279	-0.574240264551353\\
4.82882882882883	-0.582630718136389\\
4.86486486486486	-0.589999956189752\\
4.90690690690691	-0.597407049186104\\
4.94894894894895	-0.603659518158657\\
4.99099099099099	-0.60889518907555\\
5.03903903903904	-0.613805834451717\\
5.09309309309309	-0.61818424811575\\
5.15315315315315	-0.621900767169589\\
5.21921921921922	-0.624906218721583\\
5.2972972972973	-0.627379431492132\\
5.39339339339339	-0.629320793894268\\
5.51951951951952	-0.630735168806628\\
5.70570570570571	-0.631634174876371\\
6	-0.632017094511993\\
};

\addplot[area legend, draw=none, fill=blue, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
x	y\\
0	-0.838449699190176\\
0.00600600600600601	-0.838517340302347\\
0.012012012012012	-0.838587206199224\\
0.018018018018018	-0.838659365526035\\
0.024024024024024	-0.838733888821734\\
0.03003003003003	-0.83881084855951\\
0.036036036036036	-0.838890319187488\\
0.042042042042042	-0.838972377169584\\
0.048048048048048	-0.839057101026443\\
0.0540540540540541	-0.839144571376419\\
0.0600600600600601	-0.839234870976533\\
0.0660660660660661	-0.839328084763344\\
0.0720720720720721	-0.839424299893663\\
0.0780780780780781	-0.839523605785042\\
0.0840840840840841	-0.839626094155942\\
0.0900900900900901	-0.839731859065521\\
0.0960960960960961	-0.839840996952928\\
0.102102102102102	-0.839953606676018\\
0.108108108108108	-0.840069789549386\\
0.114114114114114	-0.8401896493816\\
0.12012012012012	-0.840313292511534\\
0.126126126126126	-0.84044082784366\\
0.132132132132132	-0.840572366882181\\
0.138138138138138	-0.840708023763858\\
0.144144144144144	-0.840847915289388\\
0.15015015015015	-0.840992160953181\\
0.156156156156156	-0.841140882971362\\
0.162162162162162	-0.841294206307838\\
0.168168168168168	-0.841452258698232\\
0.174174174174174	-0.841615170671503\\
0.18018018018018	-0.841783075569051\\
0.186186186186186	-0.841956109561079\\
0.192192192192192	-0.842134411660002\\
0.198198198198198	-0.842318123730656\\
0.204204204204204	-0.842507390497076\\
0.21021021021021	-0.842702359545556\\
0.216216216216216	-0.842903181323748\\
0.222222222222222	-0.843110009135494\\
0.228228228228228	-0.843322999131103\\
0.234234234234234	-0.843542310292749\\
0.24024024024024	-0.843768104414686\\
0.246246246246246	-0.84400054607791\\
0.252252252252252	-0.844239802618934\\
0.258258258258258	-0.844486044092297\\
0.264264264264264	-0.844739443226418\\
0.27027027027027	-0.845000175372401\\
0.276276276276276	-0.845268418445363\\
0.282282282282282	-0.845544352857853\\
0.288288288288288	-0.845828161444915\\
0.294294294294294	-0.846120029380321\\
0.3003003003003	-0.846420144083485\\
0.306306306306306	-0.846728695116563\\
0.312312312312312	-0.847045874071209\\
0.318318318318318	-0.847371874444456\\
0.324324324324324	-0.847706891503155\\
0.33033033033033	-0.848051122136401\\
0.336336336336336	-0.848404764695365\\
0.342342342342342	-0.848768018819891\\
0.348348348348348	-0.849141085251268\\
0.354354354354354	-0.84952416563049\\
0.36036036036036	-0.849917462281371\\
0.366366366366366	-0.850321177977818\\
0.372372372372372	-0.850735515694562\\
0.378378378378378	-0.851160678340639\\
0.384384384384384	-0.851596868474883\\
0.39039039039039	-0.852044288002681\\
0.396396396396396	-0.852503137853242\\
0.402402402402402	-0.852973617636583\\
0.408408408408408	-0.853455925279455\\
0.414414414414414	-0.853950256639405\\
0.42042042042042	-0.854456805096151\\
0.426426426426426	-0.85497576111946\\
0.432432432432432	-0.855507311812683\\
0.438438438438438	-0.856051640431106\\
0.444444444444444	-0.856608925874281\\
0.45045045045045	-0.857179342151475\\
0.456456456456456	-0.857763057819384\\
0.462462462462462	-0.858360235391259\\
0.468468468468468	-0.858971030716593\\
0.474474474474474	-0.859595592330514\\
0.48048048048048	-0.860234060772041\\
0.486486486486487	-0.860886567870377\\
0.492492492492492	-0.861553235998404\\
0.498498498498498	-0.862234177292579\\
0.504504504504504	-0.862929492838444\\
0.510510510510511	-0.863639271820972\\
0.516516516516517	-0.864363590639015\\
0.522522522522523	-0.865102511983132\\
0.528528528528528	-0.865856083876123\\
0.534534534534535	-0.866624338675619\\
0.540540540540541	-0.867407292038126\\
0.546546546546547	-0.868204941843977\\
0.552552552552553	-0.869017267082676\\
0.558558558558559	-0.869844226698199\\
0.564564564564565	-0.87068575839387\\
0.570570570570571	-0.871541777396488\\
0.576576576576577	-0.872412175179488\\
0.582582582582583	-0.873296818144965\\
0.588588588588589	-0.874195546264507\\
0.594594594594595	-0.875108171678868\\
0.600600600600601	-0.876034477256621\\
0.606606606606607	-0.876974215112035\\
0.612612612612613	-0.877927105082573\\
0.618618618618619	-0.878892833166488\\
0.624624624624625	-0.879871049921193\\
0.630630630630631	-0.880861368823181\\
0.636636636636637	-0.881863364590484\\
0.642642642642643	-0.882876571468782\\
0.648648648648649	-0.883900481482505\\
0.654654654654655	-0.884934542652436\\
0.660660660660661	-0.88597815718156\\
0.666666666666667	-0.887030679611119\\
0.672672672672673	-0.888091414949061\\
0.678678678678679	-0.889159616773367\\
0.684684684684685	-0.890234485312963\\
0.690690690690691	-0.891315165509257\\
0.696696696696697	-0.892400745061632\\
0.702702702702703	-0.893490252460549\\
0.708708708708709	-0.894582655012279\\
0.714714714714715	-0.895676856859636\\
0.720720720720721	-0.896771697003503\\
0.726726726726727	-0.897865947330317\\
0.732732732732733	-0.898958310651167\\
0.738738738738739	-0.900047418758608\\
0.744744744744745	-0.901131830507772\\
0.750750750750751	-0.902210029928917\\
0.756756756756757	-0.903280424379097\\
0.762762762762763	-0.904341342741206\\
0.768768768768769	-0.90539103367931\\
0.774774774774775	-0.906427663959804\\
0.780780780780781	-0.907449316848649\\
0.786786786786787	-0.908453990595669\\
0.792792792792793	-0.909439597017664\\
0.798798798798799	-0.910403960192928\\
0.804804804804805	-0.911344815280597\\
0.810810810810811	-0.912259807479188\\
0.816816816816817	-0.913146491139651\\
0.822822822822823	-0.914002329049238\\
0.828828828828829	-0.91482469190359\\
0.834834834834835	-0.915610857985544\\
0.840840840840841	-0.916358013070355\\
0.846846846846847	-0.917063250578235\\
0.852852852852853	-0.917723571996451\\
0.858858858858859	-0.918335887594563\\
0.864864864864865	-0.918897017457807\\
0.870870870870871	-0.919403692865164\\
0.876876876876877	-0.919852558040187\\
0.882882882882883	-0.920240172304328\\
0.888888888888889	-0.920563012664235\\
0.894894894894895	-0.920817476866266\\
0.900900900900901	-0.920999886953383\\
0.906906906906907	-0.921106493361525\\
0.912912912912913	-0.921133479594648\\
0.918918918918919	-0.921076967519731\\
0.924924924924925	-0.920933023325306\\
0.930930930930931	-0.920697664189414\\
0.936936936936937	-0.920366865705275\\
0.942942942942943	-0.919936570115562\\
0.948948948948949	-0.919402695408758\\
0.954954954954955	-0.918761145333858\\
0.960960960960961	-0.918007820392563\\
0.966966966966967	-0.917138629871081\\
0.972972972972973	-0.916149504976824\\
0.978978978978979	-0.915036413148563\\
0.984984984984985	-0.91379537361202\\
0.990990990990991	-0.912422474256537\\
0.996996996996997	-0.910913889912247\\
1.003003003003	-0.909265902111196\\
1.00900900900901	-0.907474920420219\\
1.01501501501502	-0.905537505437859\\
1.02102102102102	-0.903450393552663\\
1.02702702702703	-0.901210523565436\\
1.03303303303303	-0.898815065283936\\
1.03903903903904	-0.896261450204919\\
1.04504504504505	-0.893547404405581\\
1.05105105105105	-0.890670983774551\\
1.05705705705706	-0.887630611721743\\
1.06306306306306	-0.884425119516917\\
1.06906906906907	-0.881053789419187\\
1.07507507507508	-0.877516400774159\\
1.08108108108108	-0.873813279272976\\
1.08708708708709	-0.869945349589018\\
1.09309309309309	-0.865914191635598\\
1.0990990990991	-0.861722100726464\\
1.10510510510511	-0.857372151984062\\
1.11111111111111	-0.852868269484481\\
1.11711711711712	-0.848215301156168\\
1.12312312312312	-0.843419104035532\\
1.12912912912913	-0.838486727251383\\
1.13513513513514	-0.839484314941669\\
1.14114114114114	-0.844390087978633\\
1.14714714714715	-0.849158141808502\\
1.15315315315315	-0.853781709006381\\
1.15915915915916	-0.858255142386236\\
1.16516516516517	-0.862573785253099\\
1.17117117117117	-0.866733889213578\\
1.17717717717718	-0.870732540577203\\
1.18318318318318	-0.874567592212406\\
1.18918918918919	-0.87823760002076\\
1.1951951951952	-0.88174176358253\\
1.2012012012012	-0.885079870644721\\
1.20720720720721	-0.888252245178827\\
1.21321321321321	-0.891259698771056\\
1.21921921921922	-0.894103485134034\\
1.22522522522523	-0.896785257549477\\
1.23123123123123	-0.899307029068248\\
1.23723723723724	-0.901671135308233\\
1.24324324324324	-0.903880199702379\\
1.24924924924925	-0.905937101059549\\
1.25525525525526	-0.907844943309744\\
1.26126126126126	-0.909607027313114\\
1.26726726726727	-0.911226824619213\\
1.27327327327327	-0.912707953069242\\
1.27927927927928	-0.914054154139755\\
1.28528528528529	-0.915269271931585\\
1.29129129129129	-0.916357233712563\\
1.2972972972973	-0.917322031927176\\
1.3033033033033	-0.918167707590512\\
1.30930930930931	-0.918898334987837\\
1.31531531531532	-0.919518007604932\\
1.32132132132132	-0.920030825217891\\
1.32732732732733	-0.920440882074487\\
1.33333333333333	-0.920752256102476\\
1.33933933933934	-0.920968999083316\\
1.34534534534535	-0.921095127732744\\
1.35135135135135	-0.921134615632521\\
1.35735735735736	-0.921091385960378\\
1.36336336336336	-0.920969304967828\\
1.36936936936937	-0.920772176158014\\
1.37537537537538	-0.920503735118184\\
1.38138138138138	-0.920167644963693\\
1.38738738738739	-0.919767492352658\\
1.39339339339339	-0.919306784032507\\
1.3993993993994	-0.918788943881717\\
1.40540540540541	-0.918217310411964\\
1.41141141141141	-0.917595134697805\\
1.41741741741742	-0.916925578702775\\
1.42342342342342	-0.916211713972494\\
1.42942942942943	-0.915456520667016\\
1.43543543543544	-0.914662886906215\\
1.44144144144144	-0.913833608403471\\
1.44744744744745	-0.912971388364354\\
1.45345345345345	-0.912078837628351\\
1.45945945945946	-0.911158475032956\\
1.46546546546547	-0.910212727980694\\
1.47147147147147	-0.90924393319079\\
1.47747747747748	-0.908254337618306\\
1.48348348348348	-0.907246099524651\\
1.48948948948949	-0.906221289684326\\
1.4954954954955	-0.905181892713745\\
1.5015015015015	-0.904129808508875\\
1.50750750750751	-0.90306685377927\\
1.51351351351351	-0.90199476366691\\
1.51951951951952	-0.900915193439011\\
1.52552552552553	-0.899829720244693\\
1.53153153153153	-0.898739844926105\\
1.53753753753754	-0.897646993875218\\
1.54354354354354	-0.896552520928163\\
1.54954954954955	-0.895457709289521\\
1.55555555555556	-0.89436377347957\\
1.56156156156156	-0.89327186129797\\
1.56756756756757	-0.892183055797902\\
1.57357357357357	-0.891098377265098\\
1.57957957957958	-0.890018785196666\\
1.58558558558559	-0.888945180275015\\
1.59159159159159	-0.887878406332573\\
1.5975975975976	-0.88681925230336\\
1.6036036036036	-0.885768454157819\\
1.60960960960961	-0.884726696817641\\
1.61561561561562	-0.883694616047616\\
1.62162162162162	-0.882672800321829\\
1.62762762762763	-0.88166179266181\\
1.63363363363363	-0.880662092444466\\
1.63963963963964	-0.879674157177891\\
1.64564564564565	-0.878698404243371\\
1.65165165165165	-0.877735212602078\\
1.65765765765766	-0.876784924465198\\
1.66366366366366	-0.875847846926368\\
1.66966966966967	-0.874924253555506\\
1.67567567567568	-0.87401438595326\\
1.68168168168168	-0.873118455265455\\
1.68768768768769	-0.872236643657064\\
1.69369369369369	-0.871369105745352\\
1.6996996996997	-0.870515969991951\\
1.70570570570571	-0.869677340053774\\
1.71171171171171	-0.868853296092728\\
1.71771771771772	-0.868043896044326\\
1.72372372372372	-0.867249176845366\\
1.72972972972973	-0.866469155620913\\
1.73573573573574	-0.865703830830941\\
1.74174174174174	-0.864953183376998\\
1.74774774774775	-0.86421717766937\\
1.75375375375375	-0.863495762655257\\
1.75975975975976	-0.862788872808514\\
1.76576576576577	-0.862096429081582\\
1.77177177177177	-0.861418339820245\\
1.77777777777778	-0.860754501641922\\
1.78378378378378	-0.860104800278191\\
1.78978978978979	-0.859469111382312\\
1.7957957957958	-0.858847301302515\\
1.8018018018018	-0.858239227821843\\
1.80780780780781	-0.857644740865372\\
1.81381381381381	-0.857063683175621\\
1.81981981981982	-0.856495890956997\\
1.82582582582583	-0.855941194490115\\
1.83183183183183	-0.855399418716847\\
1.83783783783784	-0.854870383796954\\
1.84384384384384	-0.854353905637149\\
1.84984984984985	-0.853849796393456\\
1.85585585585586	-0.853357864947704\\
1.86186186186186	-0.852877917359016\\
1.86786786786787	-0.852409757291121\\
1.87387387387387	-0.85195318641632\\
1.87987987987988	-0.851508004796944\\
1.88588588588589	-0.851074011245098\\
1.89189189189189	-0.850651003661501\\
1.8978978978979	-0.850238779354206\\
1.9039039039039	-0.849837135337981\\
1.90990990990991	-0.849445868615096\\
1.91591591591592	-0.849064776438276\\
1.92192192192192	-0.848693656556545\\
1.92792792792793	-0.848332307444658\\
1.93393393393393	-0.847980528516844\\
1.93993993993994	-0.847638120325514\\
1.94594594594595	-0.847304884745605\\
1.95195195195195	-0.846980625145211\\
1.95795795795796	-0.846665146543109\\
1.96396396396396	-0.8463582557538\\
1.96996996996997	-0.846059761520657\\
1.97597597597598	-0.845769474637737\\
1.98198198198198	-0.845487208060829\\
1.98798798798799	-0.845212777008256\\
1.99399399399399	-0.844945999051962\\
2	-0.844686694199378\\
2.00600600600601	-0.844434684966548\\
2.01201201201201	-0.84418979644299\\
2.01801801801802	-0.843951856348726\\
2.02402402402402	-0.843720695083922\\
2.03003003003003	-0.843496145771556\\
2.03603603603604	-0.843278044293504\\
2.04204204204204	-0.84306622932043\\
2.04804804804805	-0.842860542335856\\
2.05405405405405	-0.842660827654754\\
2.06006006006006	-0.842466932436999\\
2.06606606606607	-0.842278706696019\\
2.07207207207207	-0.842096003302928\\
2.07807807807808	-0.841918677986466\\
2.08408408408408	-0.841746589329007\\
2.09009009009009	-0.84157959875891\\
2.0960960960961	-0.841417570539476\\
2.1021021021021	-0.841260371754754\\
2.10810810810811	-0.841107872292423\\
2.11411411411411	-0.840959944823979\\
2.12012012012012	-0.840816464782436\\
2.12612612612613	-0.840677310337743\\
2.13213213213213	-0.840542362370103\\
2.13813813813814	-0.840411504441378\\
2.14414414414414	-0.840284622764756\\
2.15015015015015	-0.840161606172826\\
2.15615615615616	-0.840042346084238\\
2.16216216216216	-0.839926736469068\\
2.16816816816817	-0.839814673813045\\
2.17417417417417	-0.839706057080755\\
2.18018018018018	-0.839600787677954\\
2.18618618618619	-0.839498769413096\\
2.19219219219219	-0.839399908458191\\
2.1981981981982	-0.839304113309084\\
2.2042042042042	-0.839211294745267\\
2.21021021021021	-0.839121365789293\\
2.21621621621622	-0.839034241665887\\
2.22222222222222	-0.838949839760836\\
2.22822822822823	-0.838868079579716\\
2.23423423423423	-0.838788882706537\\
2.24024024024024	-0.838712172762362\\
2.24624624624625	-0.838637875363961\\
2.25225225225225	-0.838565918082556\\
2.25825825825826	-0.838496230402706\\
2.26426426426426	-0.838428743681371\\
2.27027027027027	-0.838363391107215\\
2.27627627627628	-0.838300107660168\\
2.28228228228228	-0.8382388300713\\
2.28828828828829	-0.838179496783024\\
2.29429429429429	-0.838122047909675\\
2.3003003003003	-0.838066425198475\\
2.30630630630631	-0.838012571990927\\
2.31231231231231	-0.837960433184637\\
2.31831831831832	-0.837909955195613\\
2.32432432432432	-0.83786108592103\\
2.33033033033033	-0.837813774702498\\
2.33633633633634	-0.837767972289832\\
2.34234234234234	-0.837723630805345\\
2.34834834834835	-0.837680703708672\\
2.35435435435435	-0.837639145762128\\
2.36036036036036	-0.837598912996616\\
2.36636636636637	-0.837559962678084\\
2.37237237237237	-0.837522253274533\\
2.37837837837838	-0.837485744423591\\
2.38438438438438	-0.837450396900634\\
2.39039039039039	-0.837416172587481\\
2.3963963963964	-0.837383034441637\\
2.4024024024024	-0.8373509464661\\
2.40840840840841	-0.837319873679721\\
2.41441441441441	-0.83728978208812\\
2.42042042042042	-0.837260638655147\\
2.42642642642643	-0.837232411274888\\
2.43243243243243	-0.837205068744213\\
2.43843843843844	-0.837178580735855\\
2.44444444444444	-0.837152917772012\\
2.45045045045045	-0.83712805119848\\
2.45645645645646	-0.837103953159283\\
2.46246246246246	-0.837080596571822\\
2.46846846846847	-0.837057955102512\\
2.47447447447447	-0.837036003142907\\
2.48048048048048	-0.837014715786311\\
2.48648648648649	-0.836994068804851\\
2.49249249249249	-0.836974038627012\\
2.4984984984985	-0.836954602315626\\
2.5045045045045	-0.836935737546297\\
2.51051051051051	-0.836917422586261\\
2.51651651651652	-0.836899636273662\\
2.52252252252252	-0.836882357997237\\
2.52852852852853	-0.836865567676405\\
2.53453453453453	-0.83684924574174\\
2.54054054054054	-0.836833373115821\\
2.54654654654655	-0.836817931194451\\
2.55255255255255	-0.836802901828227\\
2.55855855855856	-0.836788267304457\\
2.56456456456456	-0.836774010329412\\
2.57057057057057	-0.836760114010893\\
2.57657657657658	-0.836746561841113\\
2.58258258258258	-0.836733337679876\\
2.58858858858859	-0.836720425738047\\
2.59459459459459	-0.836707810561292\\
2.6006006006006	-0.836695477014089\\
2.60660660660661	-0.836683410263987\\
2.61261261261261	-0.836671595766109\\
2.61861861861862	-0.83666001924789\\
2.62462462462462	-0.836648666694024\\
2.63063063063063	-0.836637524331632\\
2.63663663663664	-0.836626578615608\\
2.64264264264264	-0.836615816214171\\
2.64864864864865	-0.836605223994574\\
2.65465465465465	-0.836594789008981\\
2.66066066066066	-0.836584498480497\\
2.66666666666667	-0.83657433978933\\
2.67267267267267	-0.836564300459089\\
2.67867867867868	-0.83655436814319\\
2.68468468468468	-0.836544530611375\\
2.69069069069069	-0.836534775736316\\
2.6966966966967	-0.836525091480308\\
2.7027027027027	-0.836515465882028\\
2.70870870870871	-0.836505887043357\\
2.71471471471471	-0.836496343116241\\
2.72072072072072	-0.836486822289601\\
2.72672672672673	-0.836477312776255\\
2.73273273273273	-0.836467802799862\\
2.73873873873874	-0.836458280581859\\
2.74474474474474	-0.836448734328394\\
2.75075075075075	-0.836439152217237\\
2.75675675675676	-0.836429522384649\\
2.76276276276276	-0.836419832912216\\
2.76876876876877	-0.836410071813619\\
2.77477477477477	-0.836400227021333\\
2.78078078078078	-0.836390286373251\\
2.78678678678679	-0.83638023759921\\
2.79279279279279	-0.836370068307408\\
2.7987987987988	-0.83635976597071\\
2.8048048048048	-0.83634931791282\\
2.81081081081081	-0.836338711294306\\
2.81681681681682	-0.836327933098481\\
2.82282282282282	-0.836316970117099\\
2.82882882882883	-0.836305808935884\\
2.83483483483483	-0.836294435919862\\
2.84084084084084	-0.836282837198477\\
2.84684684684685	-0.836270998650497\\
2.85285285285285	-0.836258905888685\\
2.85885885885886	-0.836246544244213\\
2.86486486486486	-0.836233898750826\\
2.87087087087087	-0.836220954128726\\
2.87687687687688	-0.836207694768166\\
2.88288288288288	-0.836194104712742\\
2.88888888888889	-0.836180167642365\\
2.89489489489489	-0.836165866855905\\
2.9009009009009	-0.836151185253482\\
2.90690690690691	-0.836136105318396\\
2.91291291291291	-0.83612060909868\\
2.91891891891892	-0.83610467818826\\
2.92492492492492	-0.836088293707697\\
2.93093093093093	-0.83607143628452\\
2.93693693693694	-0.836054086033097\\
2.94294294294294	-0.836036222534064\\
2.94894894894895	-0.836017824813266\\
2.95495495495495	-0.835998871320214\\
2.96096096096096	-0.835979339906021\\
2.96696696696697	-0.835959207800825\\
2.97297297297297	-0.835938451590649\\
2.97897897897898	-0.835917047193703\\
2.98498498498498	-0.835894969836107\\
2.99099099099099	-0.835872194027001\\
2.996996996997	-0.835848693533039\\
3.003003003003	-0.835824441352239\\
3.00900900900901	-0.835799409687166\\
3.01501501501502	-0.835773569917436\\
3.02102102102102	-0.835746892571516\\
3.02702702702703	-0.835719347297791\\
3.03303303303303	-0.835690902834889\\
3.03903903903904	-0.835661526981232\\
3.04504504504505	-0.835631186563799\\
3.05105105105105	-0.83559984740606\\
3.05705705705706	-0.835567474295085\\
3.06306306306306	-0.835534030947776\\
3.06906906906907	-0.835499479976218\\
3.07507507507508	-0.835463782852107\\
3.08108108108108	-0.835426899870248\\
3.08708708708709	-0.835388790111077\\
3.09309309309309	-0.835349411402196\\
3.0990990990991	-0.835308720278884\\
3.10510510510511	-0.835266671943562\\
3.11111111111111	-0.835223220224177\\
3.11711711711712	-0.835178317531486\\
3.12312312312312	-0.835131914815201\\
3.12912912912913	-0.835083961518965\\
3.13513513513514	-0.835034405534142\\
3.14114114114114	-0.834983193152364\\
3.14714714714715	-0.834930269016831\\
3.15315315315315	-0.834875576072309\\
3.15915915915916	-0.834819055513809\\
3.16516516516517	-0.834760646733899\\
3.17117117117117	-0.834700287268623\\
3.17717717717718	-0.834637912741988\\
3.18318318318318	-0.834573456808987\\
3.18918918918919	-0.834506851097115\\
3.1951951951952	-0.834438025146342\\
3.2012012012012	-0.834366906347508\\
3.20720720720721	-0.834293419879095\\
3.21321321321321	-0.834217488642345\\
3.21921921921922	-0.834139033194672\\
3.22522522522523	-0.834057971681334\\
3.23123123123123	-0.83397421976532\\
3.23723723723724	-0.83388769055541\\
3.24324324324324	-0.833798294532364\\
3.24924924924925	-0.833705939473194\\
3.25525525525526	-0.833610530373476\\
3.26126126126126	-0.83351196936765\\
3.26726726726727	-0.833410155647267\\
3.27327327327327	-0.833304985377138\\
3.27927927927928	-0.833196351609323\\
3.28528528528529	-0.833084144194924\\
3.29129129129129	-0.832968249693627\\
3.2972972972973	-0.832848551280942\\
3.3033033033033	-0.832724928653085\\
3.30930930930931	-0.832597257929465\\
3.31531531531532	-0.832465411552702\\
3.32132132132132	-0.832329258186139\\
3.32732732732733	-0.832188662608791\\
3.33333333333333	-0.832043485607668\\
3.33933933933934	-0.831893583867431\\
3.34534534534535	-0.831738809857314\\
3.35135135135135	-0.831579011715266\\
3.35735735735736	-0.831414033129247\\
3.36336336336336	-0.831243713215638\\
3.36936936936937	-0.831067886394695\\
3.37537537537538	-0.830886382263001\\
3.38138138138138	-0.830699025462855\\
3.38738738738739	-0.83050563554855\\
3.39339339339339	-0.830306026849485\\
3.3993993993994	-0.830100008330055\\
3.40540540540541	-0.829887383446271\\
3.41141141141141	-0.829667949999056\\
3.41741741741742	-0.829441499984181\\
3.42342342342342	-0.829207819438774\\
3.42942942942943	-0.828966688284372\\
3.43543543543544	-0.828717880166476\\
3.44144144144144	-0.828461162290561\\
3.44744744744745	-0.828196295254508\\
3.45345345345345	-0.827923032877431\\
3.45945945945946	-0.827641122024867\\
3.46546546546547	-0.827350302430301\\
3.47147147147147	-0.827050306513029\\
3.47747747747748	-0.826740859192312\\
3.48348348348348	-0.82642167769785\\
3.48948948948949	-0.826092471376557\\
3.4954954954955	-0.825752941495653\\
3.5015015015015	-0.825402781042088\\
3.50750750750751	-0.825041674518328\\
3.51351351351351	-0.824669297734542\\
3.51951951951952	-0.824285317597227\\
3.52552552552553	-0.823889391894354\\
3.53153153153153	-0.823481169077082\\
3.53753753753754	-0.823060288038151\\
3.54354354354354	-0.822626377887049\\
3.54954954954955	-0.822179057722067\\
3.55555555555556	-0.821717936399397\\
3.56156156156156	-0.82124261229942\\
3.56756756756757	-0.820752673090363\\
3.57357357357357	-0.82024769548954\\
3.57957957957958	-0.819727245022388\\
3.58558558558559	-0.819190875779568\\
3.59159159159159	-0.818638130172392\\
3.5975975975976	-0.818068538686911\\
3.6036036036036	-0.817481619636983\\
3.60960960960961	-0.816876878916727\\
3.61561561561562	-0.816253809752738\\
3.62162162162162	-0.815611892456561\\
3.62762762762763	-0.81495059417787\\
3.63363363363363	-0.814269368658937\\
3.63963963963964	-0.813567655990927\\
3.64564564564565	-0.812844882372689\\
3.65165165165165	-0.812100459872707\\
3.65765765765766	-0.811333786194941\\
3.66366366366366	-0.810544244449388\\
3.66966966966967	-0.80973120292817\\
3.67567567567568	-0.808894014888112\\
3.68168168168168	-0.808032018340767\\
3.68768768768769	-0.807144535850958\\
3.69369369369369	-0.806230874344963\\
3.6996996996997	-0.805290324929546\\
3.70570570570571	-0.804322162723122\\
3.71171171171171	-0.803325646700429\\
3.71771771771772	-0.802300019552157\\
3.72372372372372	-0.801244507561083\\
3.72972972972973	-0.80015832049636\\
3.73573573573574	-0.79904065152769\\
3.74174174174174	-0.797890677161228\\
3.74774774774775	-0.796707557199156\\
3.75375375375375	-0.795490434724986\\
3.75975975975976	-0.794238436116751\\
3.76576576576577	-0.792950671090377\\
3.77177177177177	-0.791626232775611\\
3.77777777777778	-0.79026419782704\\
3.78378378378378	-0.788863626572849\\
3.78978978978979	-0.787423563204074\\
3.7957957957958	-0.785943036007252\\
3.8018018018018	-0.784421057643518\\
3.80780780780781	-0.782856625477283\\
3.81381381381381	-0.781248721957832\\
3.81981981981982	-0.779596315057253\\
3.82582582582583	-0.777898358768291\\
3.83183183183183	-0.776153793665849\\
3.83783783783784	-0.774361547535973\\
3.84384384384384	-0.772520536076359\\
3.84984984984985	-0.770629663672486\\
3.85585585585586	-0.768687824253678\\
3.86186186186186	-0.766693902233504\\
3.86786786786787	-0.764646773539057\\
3.87387387387387	-0.762545306733827\\
3.87987987987988	-0.760388364238938\\
3.88588588588589	-0.758174803657735\\
3.89189189189189	-0.755903479208731\\
3.8978978978979	-0.753573243272106\\
3.9039039039039	-0.751182948055024\\
3.90990990990991	-0.748731447381139\\
3.91591591591592	-0.746217598609737\\
3.92192192192192	-0.743640264690033\\
3.92792792792793	-0.740998316356217\\
3.93393393393393	-0.738290634468901\\
3.93993993993994	-0.735516112508586\\
3.94594594594595	-0.732673659226851\\
3.95195195195195	-0.729762201460938\\
3.95795795795796	-0.726780687117322\\
3.96396396396396	-0.723728088329878\\
3.96996996996997	-0.720603404798119\\
3.97597597597598	-0.717405667310858\\
3.98198198198198	-0.714133941460545\\
3.98798798798799	-0.710787331553257\\
3.99399399399399	-0.707364984719178\\
4	-0.703866095228094\\
4.00600600600601	-0.700289909014043\\
4.01201201201201	-0.696635728412978\\
4.01801801801802	-0.692902917116796\\
4.02402402402402	-0.689090905346573\\
4.03003003003003	-0.685199195247333\\
4.03603603603604	-0.681227366505911\\
4.04204204204204	-0.677175082192833\\
4.04804804804805	-0.67304209482826\\
4.05405405405405	-0.66882825267103\\
4.06006006006006	-0.664533506228957\\
4.06606606606607	-0.660157914987204\\
4.07207207207207	-0.655701654350346\\
4.07807807807808	-0.651165022792273\\
4.08408408408408	-0.646548449206495\\
4.09009009009009	-0.641852500447662\\
4.0960960960961	-0.637077889053177\\
4.1021021021021	-0.632225481131633\\
4.10810810810811	-0.627296304402519\\
4.11411411411411	-0.622291556369009\\
4.12012012012012	-0.617212612602878\\
4.12612612612613	-0.612061035117657\\
4.13213213213213	-0.606838580802464\\
4.13813813813814	-0.601547209885778\\
4.14414414414414	-0.596189094394009\\
4.15015015015015	-0.590766626565758\\
4.15615615615616	-0.585282427177845\\
4.16216216216216	-0.579739353734147\\
4.16816816816817	-0.574140508462988\\
4.17417417417417	-0.568489246062619\\
4.18018018018018	-0.562789181128432\\
4.18618618618619	-0.557044195188511\\
4.19219219219219	-0.551258443266832\\
4.1981981981982	-0.545436359885819\\
4.2042042042042	-0.539582664411568\\
4.21021021021021	-0.53370236563642\\
4.21621621621622	-0.52780076548422\\
4.22222222222222	-0.521883461713992\\
4.22822822822823	-0.515956349487485\\
4.23423423423423	-0.510025621655799\\
4.24024024024024	-0.504097767609284\\
4.24624624624625	-0.498179570524547\\
4.25225225225225	-0.492278102830804\\
4.25825825825826	-0.486400719708355\\
4.26426426426426	-0.480555050421406\\
4.27027027027027	-0.474748987279589\\
4.27627627627628	-0.468990672015964\\
4.28228228228228	-0.463288479367199\\
4.28828828828829	-0.457650997646526\\
4.29429429429429	-0.452087006124671\\
4.3003003003003	-0.446605449117466\\
4.30630630630631	-0.441215407035856\\
4.31231231231231	-0.435926066933694\\
4.31831831831832	-0.430746731437532\\
4.32432432432432	-0.429766287795533\\
4.33033033033033	-0.434923405805322\\
4.33633633633634	-0.44019236395004\\
4.34234234234234	-0.445563797461622\\
4.34834834834835	-0.451028501324285\\
4.35435435435435	-0.456577372482965\\
4.36036036036036	-0.462201438181953\\
4.36636636636637	-0.467891885369908\\
4.37237237237237	-0.47364008723631\\
4.37837837837838	-0.479437626459217\\
4.38438438438438	-0.485276315231895\\
4.39039039039039	-0.491148212243867\\
4.3963963963964	-0.497045636823027\\
4.4024024024024	-0.502961180453434\\
4.40840840840841	-0.508887715881181\\
4.41441441441441	-0.514818404016015\\
4.42042042042042	-0.520746698827616\\
4.42642642642643	-0.526666350426194\\
4.43243243243243	-0.532571406507045\\
4.43843843843844	-0.538456212327134\\
4.44444444444444	-0.544315409371731\\
4.45045045045045	-0.550143932858084\\
4.45645645645646	-0.555937008212319\\
4.46246246246246	-0.561690146646109\\
4.46846846846847	-0.567399139949314\\
4.47447447447447	-0.573060054605757\\
4.48048048048048	-0.578669225330557\\
4.48648648648649	-0.584223248118725\\
4.49249249249249	-0.589718972887183\\
4.4984984984985	-0.595153495785008\\
4.5045045045045	-0.6005241512395\\
4.51051051051051	-0.605828503799691\\
4.51651651651652	-0.611064339832708\\
4.52252252252252	-0.61622965912287\\
4.52852852852853	-0.621322666418418\\
4.53453453453453	-0.626341762965965\\
4.54054054054054	-0.631285538068289\\
4.54654654654655	-0.636152760697459\\
4.55255255255255	-0.640942371190875\\
4.55855855855856	-0.645653473055343\\
4.56456456456456	-0.650285324900295\\
4.57057057057057	-0.654837332519068\\
4.57657657657658	-0.659309041134145\\
4.58258258258258	-0.663700127820198\\
4.58858858858859	-0.668010394116272\\
4.59459459459459	-0.672239758836832\\
4.6006006006006	-0.676388251089276\\
4.60660660660661	-0.680456003504213\\
4.61261261261261	-0.684443245683031\\
4.61861861861862	-0.688350297866187\\
4.62462462462462	-0.692177564824362\\
4.63063063063063	-0.695925529973568\\
4.63663663663664	-0.699594749714326\\
4.64264264264264	-0.703185847994199\\
4.64864864864865	-0.706699511092193\\
4.65465465465465	-0.710136482622883\\
4.66066066066066	-0.713497558757447\\
4.66666666666667	-0.716783583658447\\
4.67267267267267	-0.719995445124498\\
4.67867867867868	-0.723134070440792\\
4.68468468468468	-0.726200422430986\\
4.69069069069069	-0.729195495705712\\
4.6966966966967	-0.732120313102712\\
4.7027027027027	-0.73497592231343\\
4.70870870870871	-0.737763392690716\\
4.71471471471471	-0.740483812232168\\
4.72072072072072	-0.743138284733551\\
4.72672672672673	-0.7457279271067\\
4.73273273273273	-0.748253866856203\\
4.73873873873874	-0.750717239709235\\
4.74474474474474	-0.753119187392842\\
4.75075075075075	-0.755460855553067\\
4.75675675675676	-0.757743391810291\\
4.76276276276276	-0.759967943945282\\
4.76876876876877	-0.762135658210447\\
4.77477477477477	-0.764247677760947\\
4.78078078078078	-0.766305141200353\\
4.78678678678679	-0.768309181235651\\
4.79279279279279	-0.770260923436552\\
4.7987987987988	-0.77216148509412\\
4.8048048048048	-0.774011974173887\\
4.81081081081081	-0.775813488358741\\
4.81681681681682	-0.777567114177025\\
4.82282282282282	-0.779273926211384\\
4.82882882882883	-0.780934986384075\\
4.83483483483483	-0.782551343314547\\
4.84084084084084	-0.784124031745288\\
4.84684684684685	-0.785654072032044\\
4.85285285285285	-0.787142469694649\\
4.85885885885886	-0.788590215024889\\
4.86486486486486	-0.78999828274791\\
4.87087087087087	-0.791367631733842\\
4.87687687687688	-0.792699204756465\\
4.88288288288288	-0.793993928295837\\
4.88888888888889	-0.795252712381973\\
4.89489489489489	-0.796476450476782\\
4.9009009009009	-0.797666019391576\\
4.90690690690691	-0.798822279237632\\
4.91291291291291	-0.799946073407371\\
4.91891891891892	-0.801038228583855\\
4.92492492492492	-0.80209955477642\\
4.93093093093093	-0.803130845380364\\
4.93693693693694	-0.804132877258728\\
4.94294294294294	-0.805106410844311\\
4.94894894894895	-0.806052190260156\\
4.95495495495495	-0.806970943456855\\
4.96096096096096	-0.807863382365099\\
4.96696696696697	-0.808730203062005\\
4.97297297297297	-0.809572085949829\\
4.97897897897898	-0.810389695945775\\
4.98498498498498	-0.811183682681663\\
4.99099099099099	-0.811954680712321\\
4.996996996997	-0.812703309731632\\
5.003003003003	-0.813430174795239\\
5.00900900900901	-0.814135866548959\\
5.01501501501502	-0.814820961462071\\
5.02102102102102	-0.815486022064636\\
5.02702702702703	-0.816131597188127\\
5.03303303303303	-0.816758222208655\\
5.03903903903904	-0.817366419292173\\
5.04504504504505	-0.817956697641041\\
5.05105105105105	-0.81852955374142\\
5.05705705705706	-0.819085471610996\\
5.06306306306306	-0.819624923046567\\
5.06906906906907	-0.820148367871067\\
5.07507507507508	-0.820656254179663\\
5.08108108108108	-0.821149018584554\\
5.08708708708709	-0.821627086458162\\
5.09309309309309	-0.822090872174436\\
5.0990990990991	-0.822540779347995\\
5.10510510510511	-0.822977201070896\\
5.11111111111111	-0.823400520146801\\
5.11711711711712	-0.823811109322373\\
5.12312312312312	-0.824209331515731\\
5.12912912912913	-0.824595540041827\\
5.13513513513514	-0.824970078834608\\
5.14114114114114	-0.825333282665876\\
5.14714714714715	-0.825685477360733\\
5.15315315315315	-0.826026980009548\\
5.15915915915916	-0.826358099176379\\
5.16516516516517	-0.8266791351038\\
5.17117117117117	-0.826990379914087\\
5.17717717717718	-0.827292117806742\\
5.18318318318318	-0.827584625252338\\
5.18918918918919	-0.827868171182653\\
5.1951951951952	-0.828143017177124\\
5.2012012012012	-0.828409417645592\\
5.20720720720721	-0.828667620007371\\
5.21321321321321	-0.828917864866649\\
5.21921921921922	-0.82916038618424\\
5.22522522522523	-0.829395411445723\\
5.23123123123123	-0.829623161825988\\
5.23723723723724	-0.829843852350239\\
5.24324324324324	-0.83005769205147\\
5.24924924924925	-0.830264884124474\\
5.25525525525526	-0.830465626076429\\
5.26126126126126	-0.830660109874086\\
5.26726726726727	-0.830848522087632\\
5.27327327327327	-0.831031044031264\\
5.27927927927928	-0.831207851900528\\
5.28528528528529	-0.83137911690647\\
5.29129129129129	-0.831545005406666\\
5.2972972972973	-0.831705679033166\\
5.3033033033033	-0.831861294817422\\
5.30930930930931	-0.832012005312249\\
5.31531531531532	-0.832157958710866\\
5.32132132132132	-0.83229929896309\\
5.32732732732733	-0.832436165888719\\
5.33333333333333	-0.832568695288174\\
5.33933933933934	-0.832697019050441\\
5.34534534534535	-0.832821265258383\\
5.35135135135135	-0.832941558291463\\
5.35735735735736	-0.833058018925936\\
5.36336336336336	-0.833170764432561\\
5.36936936936937	-0.833279908671899\\
5.37537537537538	-0.83338556218722\\
5.38138138138138	-0.833487832295106\\
5.38738738738739	-0.833586823173768\\
5.39339339339339	-0.83368263594915\\
5.3993993993994	-0.83377536877886\\
5.40540540540541	-0.833865116933969\\
5.41141141141141	-0.833951972878743\\
5.41741741741742	-0.834036026348342\\
5.42342342342342	-0.834117364424531\\
5.42942942942943	-0.834196071609456\\
5.43543543543544	-0.834272229897529\\
5.44144144144144	-0.834345918845455\\
5.44744744744745	-0.834417215640457\\
5.45345345345345	-0.83448619516673\\
5.45945945945946	-0.834552930070179\\
5.46546546546547	-0.834617490821459\\
5.47147147147147	-0.834679945777384\\
5.47747747747748	-0.834740361240722\\
5.48348348348348	-0.834798801518422\\
5.48948948948949	-0.834855328978315\\
5.4954954954955	-0.834910004104316\\
5.5015015015015	-0.834962885550169\\
5.50750750750751	-0.835014030191769\\
5.51351351351351	-0.835063493178094\\
5.51951951951952	-0.83511132798078\\
5.52552552552553	-0.835157586442376\\
5.53153153153153	-0.835202318823302\\
5.53753753753754	-0.835245573847558\\
5.54354354354354	-0.835287398747192\\
5.54954954954955	-0.835327839305578\\
5.55555555555556	-0.83536693989952\\
5.56156156156156	-0.835404743540218\\
5.56756756756757	-0.835441291913123\\
5.57357357357357	-0.8354766254167\\
5.57957957957958	-0.835510783200144\\
5.58558558558559	-0.835543803200058\\
5.59159159159159	-0.835575722176121\\
5.5975975975976	-0.835606575745788\\
5.6036036036036	-0.835636398418021\\
5.60960960960961	-0.835665223626098\\
5.61561561561562	-0.835693083759507\\
5.62162162162162	-0.835720010194961\\
5.62762762762763	-0.83574603332654\\
5.63363363363363	-0.835771182595007\\
5.63963963963964	-0.835795486516291\\
5.64564564564565	-0.835818972709179\\
5.65165165165165	-0.83584166792223\\
5.65765765765766	-0.835863598059928\\
5.66366366366366	-0.835884788208097\\
5.66966966966967	-0.835905262658603\\
5.67567567567568	-0.835925044933347\\
5.68168168168168	-0.835944157807583\\
5.68768768768769	-0.835962623332566\\
5.69369369369369	-0.835980462857559\\
5.6996996996997	-0.835997697051205\\
5.70570570570571	-0.83601434592229\\
5.71171171171171	-0.836030428839904\\
5.71771771771772	-0.836045964553027\\
5.72372372372372	-0.836060971209544\\
5.72972972972973	-0.836075466374711\\
5.73573573573574	-0.836089467049089\\
5.74174174174174	-0.83610298968595\\
5.74774774774775	-0.836116050208179\\
5.75375375375375	-0.836128664024681\\
5.75975975975976	-0.836140846046313\\
5.76576576576577	-0.836152610701338\\
5.77177177177177	-0.836163971950435\\
5.77777777777778	-0.83617494330126\\
5.78378378378378	-0.836185537822579\\
5.78978978978979	-0.836195768157984\\
5.7957957957958	-0.836205646539199\\
5.8018018018018	-0.836215184798996\\
5.80780780780781	-0.836224394383718\\
5.81381381381381	-0.836233286365434\\
5.81981981981982	-0.836241871453734\\
5.82582582582583	-0.836250160007158\\
5.83183183183183	-0.836258162044296\\
5.83783783783784	-0.836265887254542\\
5.84384384384384	-0.836273345008534\\
5.84984984984985	-0.836280544368269\\
5.85585585585586	-0.836287494096921\\
5.86186186186186	-0.836294202668352\\
5.86786786786787	-0.836300678276339\\
5.87387387387387	-0.836306928843522\\
5.87987987987988	-0.836312962030075\\
5.88588588588589	-0.83631878524211\\
5.89189189189189	-0.836324405639833\\
5.8978978978979	-0.836329830145436\\
5.9039039039039	-0.83633506545076\\
5.90990990990991	-0.836340118024711\\
5.91591591591592	-0.836344994120457\\
5.92192192192192	-0.836349699782389\\
5.92792792792793	-0.836354240852885\\
5.93393393393393	-0.836358622978845\\
5.93993993993994	-0.836362851618037\\
5.94594594594595	-0.836366932045238\\
5.95195195195195	-0.836370869358186\\
5.95795795795796	-0.836374668483343\\
5.96396396396396	-0.836378334181486\\
5.96996996996997	-0.836381871053111\\
5.97597597597598	-0.836385283543677\\
5.98198198198198	-0.836388575948677\\
5.98798798798799	-0.836391752418559\\
5.99399399399399	-0.836394816963481\\
6	-0.836397773457922\\
6	-0.427636415566065\\
5.99399399399399	-0.427633461417179\\
5.98798798798799	-0.427630399393707\\
5.98198198198198	-0.427627225634241\\
5.97597597597598	-0.427623936142653\\
5.96996996996997	-0.427620526783562\\
5.96396396396396	-0.427616993277641\\
5.95795795795796	-0.42761333119679\\
5.95195195195195	-0.42760953595914\\
5.94594594594595	-0.427605602823909\\
5.93993993993994	-0.42760152688609\\
5.93393393393393	-0.427597303070973\\
5.92792792792793	-0.427592926128489\\
5.92192192192192	-0.427588390627383\\
5.91591591591592	-0.427583690949201\\
5.90990990990991	-0.427578821282089\\
5.9039039039039	-0.427573775614395\\
5.8978978978979	-0.42756854772808\\
5.89189189189189	-0.427563131191916\\
5.88588588588589	-0.427557519354478\\
5.87987987987988	-0.427551705336921\\
5.87387387387387	-0.427545682025534\\
5.86786786786787	-0.427539442064062\\
5.86186186186186	-0.4275329778458\\
5.85585585585586	-0.42752628150544\\
5.84984984984985	-0.42751934491068\\
5.84384384384384	-0.427512159653568\\
5.83783783783784	-0.427504717041594\\
5.83183183183183	-0.427497008088511\\
5.82582582582583	-0.427489023504888\\
5.81981981981982	-0.427480753688366\\
5.81381381381381	-0.42747218871365\\
5.80780780780781	-0.42746331832218\\
5.8018018018018	-0.427454131911517\\
5.7957957957958	-0.427444618524412\\
5.78978978978979	-0.427434766837553\\
5.78378378378378	-0.427424565149993\\
5.77777777777778	-0.427414001371238\\
5.77177177177177	-0.427403063008996\\
5.76576576576577	-0.427391737156576\\
5.75975975975976	-0.42738001047993\\
5.75375375375375	-0.427367869204321\\
5.74774774774775	-0.427355299100628\\
5.74174174174174	-0.42734228547126\\
5.73573573573574	-0.427328813135678\\
5.72972972972973	-0.427314866415522\\
5.72372372372372	-0.427300429119323\\
5.71771771771772	-0.427285484526804\\
5.71171171171171	-0.427270015372752\\
5.70570570570571	-0.427254003830452\\
5.6996996996997	-0.427237431494686\\
5.69369369369369	-0.42722027936427\\
5.68768768768769	-0.427202527824142\\
5.68168168168168	-0.427184156626971\\
5.67567567567568	-0.427165144874294\\
5.66966966966967	-0.427145470997164\\
5.66366366366366	-0.42712511273631\\
5.65765765765766	-0.427104047121786\\
5.65165165165165	-0.427082250452116\\
5.64564564564565	-0.42705969827292\\
5.63963963963964	-0.42703636535501\\
5.63363363363363	-0.427012225671958\\
5.62762762762763	-0.426987252377122\\
5.62162162162162	-0.426961417780123\\
5.61561561561562	-0.426934693322768\\
5.60960960960961	-0.426907049554417\\
5.6036036036036	-0.426878456106779\\
5.5975975975976	-0.426848881668138\\
5.59159159159159	-0.426818293957008\\
5.58558558558559	-0.426786659695198\\
5.57957957957958	-0.426753944580302\\
5.57357357357357	-0.426720113257594\\
5.56756756756757	-0.426685129291339\\
5.56156156156156	-0.426648955135509\\
5.55555555555556	-0.426611552103906\\
5.54954954954955	-0.426572880339694\\
5.54354354354354	-0.426532898784339\\
5.53753753753754	-0.426491565145955\\
5.53153153153153	-0.426448835867072\\
5.52552552552553	-0.426404666091808\\
5.51951951951952	-0.426359009632476\\
5.51351351351351	-0.426311818935608\\
5.50750750750751	-0.42626304504743\\
5.5015015015015	-0.426212637578768\\
5.4954954954955	-0.426160544669424\\
5.48948948948949	-0.426106712952015\\
5.48348348348348	-0.426051087515302\\
5.47747747747748	-0.42599361186702\\
5.47147147147147	-0.425934227896228\\
5.46546546546547	-0.425872875835201\\
5.45945945945946	-0.425809494220885\\
5.45345345345345	-0.425744019855953\\
5.44744744744745	-0.425676387769468\\
5.44144144144144	-0.425606531177203\\
5.43543543543544	-0.425534381441647\\
5.42942942942943	-0.425459868031732\\
5.42342342342342	-0.425382918482319\\
5.41741741741742	-0.425303458353502\\
5.41141141141141	-0.425221411189754\\
5.40540540540541	-0.425136698478987\\
5.3993993993994	-0.425049239611573\\
5.39339339339339	-0.424958951839384\\
5.38738738738739	-0.424865750234924\\
5.38138138138138	-0.42476954765061\\
5.37537537537538	-0.42467025467829\\
5.36936936936937	-0.42456777960906\\
5.36336336336336	-0.424462028393487\\
5.35735735735736	-0.424352904602305\\
5.35135135135135	-0.424240309387703\\
5.34534534534535	-0.424124141445283\\
5.33933933933934	-0.424004296976827\\
5.33333333333333	-0.423880669653956\\
5.32732732732733	-0.423753150582839\\
5.32132132132132	-0.423621628270051\\
5.31531531531532	-0.423485988589742\\
5.30930930930931	-0.42334611475225\\
5.3033033033033	-0.423201887274322\\
5.2972972972973	-0.423053183951098\\
5.29129129129129	-0.422899879830044\\
5.28528528528529	-0.422741847187\\
5.27927927927928	-0.422578955504554\\
5.27327327327327	-0.422411071452929\\
5.26726726726727	-0.422238058873604\\
5.26126126126126	-0.422059778765898\\
5.25525525525526	-0.421876089276738\\
5.24924924924925	-0.42168684569388\\
5.24324324324324	-0.421491900442821\\
5.23723723723724	-0.421291103087689\\
5.23123123123123	-0.421084300336391\\
5.22522522522523	-0.420871336050319\\
5.21921921921922	-0.420652051258926\\
5.21321321321321	-0.420426284179496\\
5.20720720720721	-0.420193870242452\\
5.2012012012012	-0.419954642122561\\
5.1951951951952	-0.419708429776396\\
5.18918918918919	-0.419455060486451\\
5.18318318318318	-0.419194358912312\\
5.17717717717718	-0.418926147149294\\
5.17117117117117	-0.418650244794988\\
5.16516516516517	-0.418366469024164\\
5.15915915915916	-0.418074634672501\\
5.15315315315315	-0.417774554329631\\
5.14714714714715	-0.417466038442\\
5.14114114114114	-0.417148895426067\\
5.13513513513514	-0.416822931792379\\
5.12912912912913	-0.416487952281083\\
5.12312312312312	-0.416143760009445\\
5.11711711711712	-0.415790156631972\\
5.11111111111111	-0.415426942513753\\
5.10510510510511	-0.415053916917635\\
5.0990990990991	-0.414670878205895\\
5.09309309309309	-0.414277624057064\\
5.08708708708709	-0.413873951698592\\
5.08108108108108	-0.413459658156039\\
5.07507507507508	-0.413034540519528\\
5.06906906906907	-0.412598396228174\\
5.06306306306306	-0.412151023373249\\
5.05705705705706	-0.411692221020833\\
5.05105105105105	-0.411221789554743\\
5.04504504504505	-0.410739531040516\\
5.03903903903904	-0.410245249611261\\
5.03303303303303	-0.40973875187618\\
5.02702702702703	-0.4092198473526\\
5.02102102102102	-0.408688348922332\\
5.01501501501502	-0.408144073313215\\
5.00900900900901	-0.407586841606674\\
5.003003003003	-0.407016479772163\\
4.996996996997	-0.406432819229331\\
4.99099099099099	-0.40583569743878\\
4.98498498498498	-0.405224958522252\\
4.97897897897898	-0.404600453913109\\
4.97297297297297	-0.403962043037952\\
4.96696696696697	-0.403309594030187\\
4.96096096096096	-0.4026429844764\\
4.95495495495495	-0.401962102196319\\
4.94894894894895	-0.401266846057158\\
4.94294294294294	-0.400557126823126\\
4.93693693693694	-0.399832868040835\\
4.93093093093093	-0.399094006961309\\
4.92492492492492	-0.398340495499305\\
4.91891891891892	-0.397572301230561\\
4.91291291291291	-0.396789408427591\\
4.90690690690691	-0.395991819134574\\
4.9009009009009	-0.395179554281842\\
4.89489489489489	-0.394352654840417\\
4.88888888888889	-0.393511183016969\\
4.88288288288288	-0.392655223489513\\
4.87687687687688	-0.391784884684086\\
4.87087087087087	-0.390900300092552\\
4.86486486486486	-0.390001629631595\\
4.85885885885886	-0.389089061042883\\
4.85285285285285	-0.388162811334245\\
4.84684684684685	-0.38722312826162\\
4.84084084084084	-0.386270291851403\\
4.83483483483483	-0.38530461596268\\
4.82882882882883	-0.384326449888702\\
4.82282282282282	-0.3833361799968\\
4.81681681681682	-0.382334231405787\\
4.81081081081081	-0.38132106969969\\
4.8048048048048	-0.380297202676514\\
4.7987987987988	-0.379263182130501\\
4.79279279279279	-0.378219605666155\\
4.78678678678679	-0.377167118542068\\
4.78078078078078	-0.376106415542363\\
4.77477477477477	-0.375038242873271\\
4.76876876876877	-0.373963400082128\\
4.76276276276276	-0.372882741995767\\
4.75675675675676	-0.371797180674965\\
4.75075075075075	-0.370707687381303\\
4.74474474474474	-0.369615294552399\\
4.73873873873874	-0.368521097781172\\
4.73273273273273	-0.367426257794336\\
4.72672672672673	-0.366332002424939\\
4.72072072072072	-0.365239628573333\\
4.71471471471471	-0.364150504150444\\
4.70870870870871	-0.363066069996776\\
4.7027027027027	-0.361987841770006\\
4.6966966966967	-0.360917411793492\\
4.69069069069069	-0.359856450857442\\
4.68468468468468	-0.358806709963833\\
4.67867867867868	-0.357770022005546\\
4.67267267267267	-0.356748303369463\\
4.66666666666667	-0.355743555452556\\
4.66066066066066	-0.354757866079199\\
4.65465465465465	-0.353793410807146\\
4.64864864864865	-0.352852454108717\\
4.64264264264264	-0.351937350412867\\
4.63663663663664	-0.351050544992806\\
4.63063063063063	-0.350194574682861\\
4.62462462462462	-0.349372068407212\\
4.61861861861862	-0.348585747501964\\
4.61261261261261	-0.34783842581091\\
4.60660660660661	-0.347133009534051\\
4.6006006006006	-0.346472496806655\\
4.59459459459459	-0.34585997698528\\
4.58858858858859	-0.345298629615753\\
4.58258258258258	-0.344791723056579\\
4.57657657657658	-0.344342612729706\\
4.57057057057057	-0.343954738968923\\
4.56456456456456	-0.343631624434415\\
4.55855855855856	-0.343376871060248\\
4.55255255255255	-0.343194156499617\\
4.54654654654655	-0.343087230030771\\
4.54054054054054	-0.343059907884448\\
4.53453453453453	-0.343116067951507\\
4.52852852852853	-0.343259643827216\\
4.52252252252252	-0.343494618146333\\
4.51651651651652	-0.343825015160643\\
4.51051051051051	-0.344254892508133\\
4.5045045045045	-0.344788332120297\\
4.4984984984985	-0.345429430211335\\
4.49249249249249	-0.346182286290114\\
4.48648648648649	-0.34705099113278\\
4.48048048048048	-0.348039613650752\\
4.47447447447447	-0.349152186585542\\
4.46846846846847	-0.350392690958451\\
4.46246246246246	-0.351765039199502\\
4.45645645645646	-0.353273056876205\\
4.45045045045045	-0.354920462938727\\
4.44444444444444	-0.356710848393679\\
4.43843843843844	-0.358647653314232\\
4.43243243243243	-0.360734142089315\\
4.42642642642643	-0.362973376809229\\
4.42042042042042	-0.365368188679324\\
4.41441441441441	-0.367921147346802\\
4.40840840840841	-0.370634528018591\\
4.4024024024024	-0.373510276240346\\
4.3963963963964	-0.37654997019707\\
4.39039039039039	-0.379754780385681\\
4.38438438438438	-0.383125426497406\\
4.37837837837838	-0.386662131333179\\
4.37237237237237	-0.39036457155815\\
4.36636636636637	-0.394231825079301\\
4.36036036036036	-0.398262314803182\\
4.35435435435435	-0.402453748492272\\
4.34834834834835	-0.406803054374987\\
4.34234234234234	-0.411306312021524\\
4.33633633633634	-0.415958677473363\\
4.33033033033033	-0.42075429806075\\
4.32432432432432	-0.425686131171948\\
4.31831831831832	-0.424729613379164\\
4.31231231231231	-0.419823289031128\\
4.30630630630631	-0.415054653133624\\
4.3003003003003	-0.410430478422112\\
4.29429429429429	-0.405956416357658\\
4.28828828828829	-0.401637127538704\\
4.28228228228228	-0.397476363945137\\
4.27627627627628	-0.393477042562919\\
4.27027027027027	-0.389641313548181\\
4.26426426426426	-0.385970623771048\\
4.25825825825826	-0.382465776186487\\
4.25225225225225	-0.379126985361554\\
4.24624624624625	-0.375953929431834\\
4.24024024024024	-0.372945798724487\\
4.23423423423423	-0.370101341258988\\
4.22822822822823	-0.367418905316198\\
4.22222222222222	-0.364896479249271\\
4.21621621621622	-0.362531728696237\\
4.21021021021021	-0.360322031341731\\
4.2042042042042	-0.358264509365406\\
4.1981981981982	-0.356356059705447\\
4.19219219219219	-0.354593382257838\\
4.18618618618619	-0.35297300612491\\
4.18018018018018	-0.351491314020482\\
4.17417417417417	-0.350144564933122\\
4.16816816816817	-0.348928915143814\\
4.16216216216216	-0.347840437689451\\
4.15615615615616	-0.346875140359058\\
4.15015015015015	-0.346028982305382\\
4.14414414414414	-0.345297889350534\\
4.13813813813814	-0.344677768060573\\
4.13213213213213	-0.34416451866035\\
4.12612612612613	-0.343754046856497\\
4.12012012012012	-0.343442274633229\\
4.11411411411411	-0.343225150082475\\
4.10810810810811	-0.34309865632693\\
4.1021021021021	-0.343058819591697\\
4.0960960960961	-0.343101716477527\\
4.09009009009009	-0.343223480485991\\
4.08408408408408	-0.343420307844416\\
4.07807807807808	-0.343688462676021\\
4.07207207207207	-0.344024281558347\\
4.06606606606607	-0.344424177510873\\
4.06006006006006	-0.344884643450577\\
4.05405405405405	-0.345402255152175\\
4.04804804804805	-0.345973673747787\\
4.04204204204204	-0.346595647798961\\
4.03603603603604	-0.347265014972144\\
4.03003003003003	-0.347978703347025\\
4.02402402402402	-0.348733732385536\\
4.01801801801802	-0.349527213587698\\
4.01201201201201	-0.350356350859077\\
4.00600600600601	-0.351218440613145\\
4	-0.352110871630509\\
3.99399399399399	-0.353031124695701\\
3.98798798798799	-0.353976772030945\\
3.98198198198198	-0.354945476545221\\
3.97597597597598	-0.355934990915776\\
3.96996996996997	-0.356943156518212\\
3.96396396396396	-0.357967902220268\\
3.95795795795796	-0.359007243053478\\
3.95195195195195	-0.360059278775948\\
3.94594594594595	-0.361122192338704\\
3.93993993993994	-0.362194248267169\\
3.93393393393393	-0.363273790968642\\
3.92792792792793	-0.364359242975873\\
3.92192192192192	-0.365449103136146\\
3.91591591591592	-0.366541944754649\\
3.90990990990991	-0.367636413700286\\
3.9039039039039	-0.368731226481488\\
3.8978978978979	-0.369825168299047\\
3.89189189189189	-0.370917091082488\\
3.88588588588589	-0.372005911515964\\
3.87987987987988	-0.373090609059231\\
3.87387387387387	-0.374170223968814\\
3.86786786786787	-0.37524385532405\\
3.86186186186186	-0.376310659062332\\
3.85585585585586	-0.377369846027464\\
3.84984984984985	-0.378420680034761\\
3.84384384384384	-0.379462475956131\\
3.83783783783784	-0.380494597828127\\
3.83183183183183	-0.381516456985639\\
3.82582582582583	-0.382527510223623\\
3.81981981981982	-0.383527257989043\\
3.81381381381381	-0.384515242604919\\
3.80780780780781	-0.38549104652819\\
3.8018018018018	-0.386454290642859\\
3.7957957957958	-0.387404632589725\\
3.78978978978979	-0.388341765133778\\
3.78378378378378	-0.389265414570213\\
3.77777777777778	-0.390175339169818\\
3.77177177177177	-0.391071327664359\\
3.76576576576577	-0.391953197772443\\
3.75975975975976	-0.392820794766207\\
3.75375375375375	-0.393673990079067\\
3.74774774774775	-0.394512679954641\\
3.74174174174174	-0.395336784136865\\
3.73573573573574	-0.396146244601209\\
3.72972972972973	-0.396941024326834\\
3.72372372372372	-0.397721106109438\\
3.71771771771772	-0.398486491414453\\
3.71171171171171	-0.399237199270215\\
3.70570570570571	-0.399973265200637\\
3.6996996996997	-0.400694740196875\\
3.69369369369369	-0.401401689727427\\
3.68768768768769	-0.402094192786054\\
3.68168168168168	-0.402772340976864\\
3.67567567567568	-0.403436237635875\\
3.66966966966967	-0.404085996988345\\
3.66366366366366	-0.404721743341105\\
3.65765765765766	-0.405343610309133\\
3.65165165165165	-0.405951740075574\\
3.64564564564565	-0.406546282684388\\
3.63963963963964	-0.407127395364811\\
3.63363363363363	-0.407695241886781\\
3.62762762762763	-0.4082499919465\\
3.62162162162162	-0.408791820581265\\
3.61561561561562	-0.409320907612716\\
3.60960960960961	-0.409837437117671\\
3.6036036036036	-0.41034159692565\\
3.5975975975976	-0.410833578142276\\
3.59159159159159	-0.411313574697692\\
3.58558558558559	-0.411781782919146\\
3.57957957957958	-0.412238401126931\\
3.57357357357357	-0.412683629252835\\
3.56756756756757	-0.413117668480312\\
3.56156156156156	-0.413540720905557\\
3.55555555555556	-0.413952989218701\\
3.54954954954955	-0.414354676404359\\
3.54354354354354	-0.414745985460758\\
3.53753753753754	-0.415127119136721\\
3.53153153153153	-0.415498279685752\\
3.52552552552553	-0.415859668636533\\
3.51951951951952	-0.416211486579123\\
3.51351351351351	-0.416553932966189\\
3.50750750750751	-0.4168872059286\\
3.5015015015015	-0.417211502104745\\
3.4954954954955	-0.417527016482954\\
3.48948948948949	-0.417833942256404\\
3.48348348348348	-0.418132470689925\\
3.47747747747748	-0.418422790998143\\
3.47147147147147	-0.418705090234389\\
3.46546546546547	-0.418979553189853\\
3.45945945945946	-0.419246362302462\\
3.45345345345345	-0.419505697574973\\
3.44744744744745	-0.419757736501814\\
3.44144144144144	-0.420002654004192\\
3.43543543543544	-0.420240622373029\\
3.42942942942943	-0.420471811219291\\
3.42342342342342	-0.420696387431295\\
3.41741741741742	-0.420914515138596\\
3.41141141141141	-0.421126355682072\\
3.40540540540541	-0.42133206758983\\
3.3993993993994	-0.421531806558594\\
3.39339339339339	-0.421725725440228\\
3.38738738738739	-0.421913974233074\\
3.38138138138138	-0.42209670007779\\
3.37537537537538	-0.422274047257403\\
3.36936936936937	-0.422446157201283\\
3.36336336336336	-0.422613168492774\\
3.35735735735736	-0.422775216880225\\
3.35135135135135	-0.422932435291176\\
3.34534534534535	-0.423084953849458\\
3.33933933933934	-0.423232899894999\\
3.33333333333333	-0.423376398006112\\
3.32732732732733	-0.42351557002407\\
3.32132132132132	-0.423650535079778\\
3.31531531531532	-0.423781409622359\\
3.30930930930931	-0.423908307449484\\
3.3033033033033	-0.424031339739286\\
3.2972972972973	-0.424150615083699\\
3.29129129129129	-0.424266239523085\\
3.28528528528529	-0.424378316582003\\
3.27927927927928	-0.424486947306003\\
3.27327327327327	-0.424592230299305\\
3.26726726726727	-0.424694261763275\\
3.26126126126126	-0.424793135535559\\
3.25525525525526	-0.424888943129802\\
3.24924924924925	-0.424981773775837\\
3.24324324324324	-0.425071714460268\\
3.23723723723724	-0.425158849967356\\
3.23123123123123	-0.425243262920133\\
3.22522522522523	-0.425325033821671\\
3.21921921921922	-0.425404241096438\\
3.21321321321321	-0.425480961131678\\
3.20720720720721	-0.425555268318756\\
3.2012012012012	-0.425627235094416\\
3.1951951951952	-0.425696931981901\\
3.18918918918919	-0.425764427631878\\
3.18318318318318	-0.425829788863146\\
3.17717717717718	-0.425893080703071\\
3.17117117117117	-0.425954366427717\\
3.16516516516517	-0.426013707601638\\
3.15915915915916	-0.426071164117307\\
3.15315315315315	-0.426126794234148\\
3.14714714714715	-0.42618065461715\\
3.14114114114114	-0.426232800375038\\
3.13513513513514	-0.426283285097981\\
3.12912912912913	-0.426332160894832\\
3.12312312312312	-0.426379478429855\\
3.11711711711712	-0.426425286958965\\
3.11111111111111	-0.426469634365429\\
3.10510510510511	-0.42651256719505\\
3.0990990990991	-0.42655413069081\\
3.09309309309309	-0.42659436882696\\
3.08708708708709	-0.426633324342575\\
3.08108108108108	-0.426671038774536\\
3.07507507507508	-0.426707552489971\\
3.06906906906907	-0.426742904718123\\
3.06306306306306	-0.42677713358167\\
3.05705705705706	-0.426810276127475\\
3.05105105105105	-0.426842368356786\\
3.04504504504505	-0.426873445254876\\
3.03903903903904	-0.426903540820132\\
3.03303303303303	-0.426932688092595\\
3.02702702702703	-0.426960919181951\\
3.02102102102102	-0.426988265294996\\
3.01501501501502	-0.427014756762551\\
3.00900900900901	-0.427040423065862\\
3.003003003003	-0.427065292862475\\
2.996996996997	-0.427089394011602\\
2.99099099099099	-0.427112753598979\\
2.98498498498498	-0.427135397961227\\
2.97897897897898	-0.427157352709729\\
2.97297297297297	-0.427178642754026\\
2.96696696696697	-0.427199292324742\\
2.96096096096096	-0.427219324996049\\
2.95495495495495	-0.427238763707684\\
2.94894894894895	-0.427257630786523\\
2.94294294294294	-0.427275947967726\\
2.93693693693694	-0.427293736415458\\
2.93093093093093	-0.42731101674321\\
2.92492492492492	-0.427327809033707\\
2.91891891891892	-0.427344132858442\\
2.91291291291291	-0.427360007296825\\
2.90690690690691	-0.427375450954964\\
2.9009009009009	-0.427390481984098\\
2.89489489489489	-0.42740511809868\\
2.88888888888889	-0.427419376594131\\
2.88288288288288	-0.427433274364269\\
2.87687687687688	-0.427446827918429\\
2.87087087087087	-0.427460053398286\\
2.86486486486486	-0.42747296659439\\
2.85885885885886	-0.427485582962419\\
2.85285285285285	-0.427497917639177\\
2.84684684684685	-0.427509985458333\\
2.84084084084084	-0.427521800965915\\
2.83483483483483	-0.42753337843558\\
2.82882882882883	-0.427544731883661\\
2.82282282282282	-0.42755587508401\\
2.81681681681682	-0.427566821582637\\
2.81081081081081	-0.427577584712175\\
2.8048048048048	-0.427588177606161\\
2.7987987987988	-0.427598613213164\\
2.79279279279279	-0.427608904310754\\
2.78678678678679	-0.427619063519344\\
2.78078078078078	-0.427629103315886\\
2.77477477477477	-0.427639036047471\\
2.76876876876877	-0.427648873944811\\
2.76276276276276	-0.427658629135628\\
2.75675675675676	-0.42766831365797\\
2.75075075075075	-0.427677939473447\\
2.74474474474474	-0.427687518480413\\
2.73873873873874	-0.4276970625271\\
2.73273273273273	-0.427706583424712\\
2.72672672672673	-0.427716092960503\\
2.72072072072072	-0.427725602910834\\
2.71471471471471	-0.42773512505423\\
2.70870870870871	-0.427744671184453\\
2.7027027027027	-0.42775425312359\\
2.6966966966967	-0.427763882735182\\
2.69069069069069	-0.42777357193739\\
2.68468468468468	-0.427783332716227\\
2.67867867867868	-0.427793177138855\\
2.67267267267267	-0.427803117366964\\
2.66666666666667	-0.427813165670245\\
2.66066066066066	-0.427823334439971\\
2.65465465465465	-0.427833636202689\\
2.64864864864865	-0.427844083634055\\
2.64264264264264	-0.427854689572797\\
2.63663663663664	-0.427865467034846\\
2.63063063063063	-0.427876429227627\\
2.62462462462462	-0.427887589564537\\
2.61861861861862	-0.427898961679612\\
2.61261261261261	-0.427910559442406\\
2.60660660660661	-0.427922396973086\\
2.6006006006006	-0.427934488657763\\
2.59459459459459	-0.427946849164072\\
2.58858858858859	-0.42795949345701\\
2.58258258258258	-0.427972436815049\\
2.57657657657658	-0.427985694846545\\
2.57057057057057	-0.427999283506437\\
2.56456456456456	-0.428013219113282\\
2.55855855855856	-0.428027518366602\\
2.55255255255255	-0.4280421983646\\
2.54654654654655	-0.428057276622219\\
2.54054054054054	-0.428072771089596\\
2.53453453453453	-0.428088700170896\\
2.52852852852853	-0.428105082743566\\
2.52252252252252	-0.428121938178006\\
2.51651651651652	-0.428139286357691\\
2.51051051051051	-0.428157147699745\\
2.5045045045045	-0.428175543175992\\
2.4984984984985	-0.428194494334504\\
2.49249249249249	-0.428214023321654\\
2.48648648648649	-0.428234152904702\\
2.48048048048048	-0.428254906494922\\
2.47447447447447	-0.428276308171303\\
2.46846846846847	-0.428298382704823\\
2.46246246246246	-0.428321155583337\\
2.45645645645646	-0.428344653037079\\
2.45045045045045	-0.428368902064811\\
2.44444444444444	-0.428393930460635\\
2.43843843843844	-0.428419766841485\\
2.43243243243243	-0.428446440675332\\
2.42642642642643	-0.428473982310104\\
2.42042042042042	-0.428502423003363\\
2.41441441441441	-0.428531794952749\\
2.40840840840841	-0.428562131327218\\
2.4024024024024	-0.428593466299099\\
2.3963963963964	-0.428625835076983\\
2.39039039039039	-0.428659273939489\\
2.38438438438438	-0.428693820269909\\
2.37837837837838	-0.428729512591773\\
2.37237237237237	-0.428766390605354\\
2.36636636636637	-0.428804495225134\\
2.36036036036036	-0.42884386861827\\
2.35435435435435	-0.428884554244076\\
2.34834834834835	-0.428926596894556\\
2.34234234234234	-0.428970042736015\\
2.33633633633634	-0.429014939351767\\
2.33033033033033	-0.429061335785991\\
2.32432432432432	-0.429109282588744\\
2.31831831831832	-0.429158831862173\\
2.31231231231231	-0.429210037307955\\
2.30630630630631	-0.429262954275999\\
2.3003003003003	-0.429317639814436\\
2.29429429429429	-0.429374152720942\\
2.28828828828829	-0.429432553595412\\
2.28228228228228	-0.429492904894043\\
2.27627627627628	-0.429555270984833\\
2.27027027027027	-0.42961971820456\\
2.26426426426426	-0.429686314917255\\
2.25825825825826	-0.429755131574222\\
2.25225225225225	-0.42982624077564\\
2.24624624624625	-0.42989971733378\\
2.24024024024024	-0.429975638337885\\
2.23423423423423	-0.430054083220744\\
2.22822822822823	-0.430135133827023\\
2.22222222222222	-0.430218874483358\\
2.21621621621622	-0.430305392070299\\
2.21021021021021	-0.430394776096103\\
2.2042042042042	-0.430487118772463\\
2.1981981981982	-0.430582515092184\\
2.19219219219219	-0.430681062908873\\
2.18618618618619	-0.430782863018683\\
2.18018018018018	-0.430888019244161\\
2.17417417417417	-0.430996638520244\\
2.16816816816817	-0.431108830982459\\
2.16216216216216	-0.431224710057373\\
2.15615615615616	-0.431344392555341\\
2.15015015015015	-0.431467998765616\\
2.14414414414414	-0.43159565255385\\
2.13813813813814	-0.431727481462069\\
2.13213213213213	-0.431863616811146\\
2.12612612612613	-0.432004193805847\\
2.12012012012012	-0.43214935164249\\
2.11411411411411	-0.432299233619286\\
2.10810810810811	-0.432453987249398\\
2.1021021021021	-0.432613764376795\\
2.0960960960961	-0.432778721294936\\
2.09009009009009	-0.432949018868354\\
2.08408408408408	-0.433124822657187\\
2.07807807807808	-0.433306303044717\\
2.07207207207207	-0.433493635367961\\
2.06606606606607	-0.433687000051389\\
2.06006006006006	-0.433886582743791\\
2.05405405405405	-0.43409257445838\\
2.04804804804805	-0.434305171716155\\
2.04204204204204	-0.434524576692588\\
2.03603603603604	-0.434750997367684\\
2.03003003003003	-0.434984647679449\\
2.02402402402402	-0.435225747680824\\
2.01801801801802	-0.43547452370012\\
2.01201201201201	-0.435731208504991\\
2.00600600600601	-0.435996041469987\\
2	-0.436269268747713\\
1.99399399399399	-0.436551143443624\\
1.98798798798799	-0.436841925794479\\
1.98198198198198	-0.437141883350477\\
1.97597597597598	-0.437451291161072\\
1.96996996996997	-0.437770431964493\\
1.96396396396396	-0.43809959638095\\
1.95795795795796	-0.438439083109531\\
1.95195195195195	-0.438789199128758\\
1.94594594594595	-0.439150259900789\\
1.93993993993994	-0.439522589579216\\
1.93393393393393	-0.439906521220424\\
1.92792792792793	-0.440302396998433\\
1.92192192192192	-0.440710568423168\\
1.91591591591592	-0.441131396562053\\
1.90990990990991	-0.441565252264834\\
1.9039039039039	-0.442012516391505\\
1.8978978978979	-0.442473580043204\\
1.89189189189189	-0.442948844795913\\
1.88588588588589	-0.443438722936786\\
1.87987987987988	-0.443943637702904\\
1.87387387387387	-0.444464023522226\\
1.86786786786787	-0.445000326256487\\
1.86186186186186	-0.445553003445756\\
1.85585585585586	-0.446122524554352\\
1.84984984984985	-0.446709371217762\\
1.84384384384384	-0.447314037490198\\
1.83783783783784	-0.44793703009237\\
1.83183183183183	-0.448578868659026\\
1.82582582582583	-0.449240085985761\\
1.81981981981982	-0.449921228274575\\
1.81381381381381	-0.450622855377566\\
1.80780780780781	-0.451345541038164\\
1.8018018018018	-0.452089873129196\\
1.7957957957958	-0.452856453887046\\
1.78978978978979	-0.453645900141138\\
1.78378378378378	-0.454458843537855\\
1.77777777777778	-0.455295930757997\\
1.77177177177177	-0.456157823726789\\
1.76576576576577	-0.457045199815374\\
1.75975975975976	-0.457958752032669\\
1.75375375375375	-0.458899189206389\\
1.74774774774775	-0.459867236151923\\
1.74174174174174	-0.460863633827732\\
1.73573573573574	-0.461889139475776\\
1.72972972972973	-0.462944526745457\\
1.72372372372372	-0.4640305857994\\
1.71771771771772	-0.465148123399376\\
1.71171171171171	-0.466297962970484\\
1.70570570570571	-0.467480944641681\\
1.6996996996997	-0.468697925260589\\
1.69369369369369	-0.469949778380421\\
1.68768768768769	-0.471237394216745\\
1.68168168168168	-0.472561679571692\\
1.67567567567568	-0.473923557723079\\
1.66966966966967	-0.475323968275825\\
1.66366366366366	-0.476763866972863\\
1.65765765765766	-0.478244225462675\\
1.65165165165165	-0.479766031020399\\
1.64564564564565	-0.481330286219351\\
1.63963963963964	-0.482938008549662\\
1.63363363363363	-0.484590229980583\\
1.62762762762763	-0.486287996462885\\
1.62162162162162	-0.488032367367637\\
1.61561561561562	-0.489824414857492\\
1.60960960960961	-0.491665223186496\\
1.6036036036036	-0.493555887924266\\
1.5975975975976	-0.495497515100274\\
1.59159159159159	-0.497491220263802\\
1.58558558558559	-0.499538127455032\\
1.57957957957958	-0.501639368082577\\
1.57357357357357	-0.503796079702649\\
1.56756756756757	-0.506009404694922\\
1.56156156156156	-0.508280488830032\\
1.55555555555556	-0.51061047972356\\
1.54954954954955	-0.51300052517121\\
1.54354354354354	-0.515451771359833\\
1.53753753753754	-0.51796536094883\\
1.53153153153153	-0.520542431016419\\
1.52552552552553	-0.523184110865176\\
1.51951951951952	-0.525891519681216\\
1.51351351351351	-0.528665764041357\\
1.50750750750751	-0.531507935262583\\
1.5015015015015	-0.534419106588164\\
1.4954954954955	-0.537400330204777\\
1.48948948948949	-0.540452634085072\\
1.48348348348348	-0.543577018650196\\
1.47747747747748	-0.546774453246891\\
1.47147147147147	-0.550045872433974\\
1.46546546546547	-0.553392172073141\\
1.45945945945946	-0.556814205219328\\
1.45345345345345	-0.56031277780608\\
1.44744744744745	-0.563888644121765\\
1.44144144144144	-0.56754250207279\\
1.43543543543544	-0.571274988230483\\
1.42942942942943	-0.575086672658744\\
1.42342342342342	-0.578978053520217\\
1.41741741741742	-0.582949551459332\\
1.41141141141141	-0.58700150376135\\
1.40540540540541	-0.591134158287359\\
1.3993993993994	-0.595347667186121\\
1.39339339339339	-0.599642080384688\\
1.38738738738739	-0.604017338860929\\
1.38138138138138	-0.60847326770233\\
1.37537537537538	-0.613009568956935\\
1.36936936936937	-0.617625814283848\\
1.36336336336336	-0.622321437412472\\
1.35735735735736	-0.627095726421623\\
1.35135135135135	-0.63194781585174\\
1.34534534534535	-0.636876678665779\\
1.33933933933934	-0.641881118076933\\
1.33333333333333	-0.64695975926409\\
1.32732732732733	-0.65211104099906\\
1.32132132132132	-0.657333207212859\\
1.31531531531532	-0.662624298532047\\
1.30930930930931	-0.667982143820035\\
1.3033033033033	-0.673404351762546\\
1.2972972972973	-0.678888302541146\\
1.29129129129129	-0.684431139643701\\
1.28528528528529	-0.690029761866147\\
1.27927927927928	-0.695680815565772\\
1.27327327327327	-0.701380687232551\\
1.26726726726727	-0.707125496451856\\
1.26126126126126	-0.712911089339115\\
1.25525525525526	-0.718733032534771\\
1.24924924924925	-0.724586607856115\\
1.24324324324324	-0.730466807711351\\
1.23723723723724	-0.736368331390469\\
1.23123123123123	-0.742285582357205\\
1.22522522522523	-0.74821266667649\\
1.21921921921922	-0.75414339272227\\
1.21321321321321	-0.760071272321264\\
1.20720720720721	-0.765989523499146\\
1.2012012012012	-0.77189107500635\\
1.1951951951952	-0.777768572811172\\
1.18918918918919	-0.78361438875757\\
1.18318318318318	-0.789420631593441\\
1.17717717717718	-0.79517916058152\\
1.17117117117117	-0.800881601907318\\
1.16516516516517	-0.806519368093283\\
1.15915915915916	-0.812083680604515\\
1.15315315315315	-0.817565595747401\\
1.14714714714715	-0.822956033609403\\
1.14114114114114	-0.8282458075269\\
1.13513513513514	-0.833425615777595\\
1.12912912912913	-0.83444815659425\\
1.12312312312312	-0.829291520016709\\
1.11711711711712	-0.824023003189858\\
1.11111111111111	-0.818651972885188\\
1.10510510510511	-0.813187634501489\\
1.0990990990991	-0.807639091567804\\
1.09309309309309	-0.802015317438387\\
1.08708708708709	-0.796325125879213\\
1.08108108108108	-0.790577144518032\\
1.07507507507508	-0.784779791582961\\
1.06906906906907	-0.778941255863095\\
1.06306306306306	-0.773069479715288\\
1.05705705705706	-0.767172144910667\\
1.05105105105105	-0.761256661106615\\
1.04504504504505	-0.755330156731289\\
1.03903903903904	-0.749399472073421\\
1.03303303303303	-0.743471154378129\\
1.02702702702703	-0.737551454759134\\
1.02102102102102	-0.731646326747976\\
1.01501501501502	-0.725761426311628\\
1.00900900900901	-0.719902113180768\\
1.003003003003	-0.714073453341643\\
0.996996996996997	-0.708280222555131\\
0.990990990990991	-0.702526910776687\\
0.984984984984985	-0.696817727360679\\
0.978978978978979	-0.69115660694199\\
0.972972972972973	-0.685547215896545\\
0.966966966966967	-0.679992959290852\\
0.960960960960961	-0.674496988238436\\
0.954954954954955	-0.669062207588441\\
0.948948948948949	-0.663691283878556\\
0.942942942942943	-0.658386653490784\\
0.936936936936937	-0.653150530954612\\
0.930930930930931	-0.647984917347583\\
0.924924924924925	-0.642891608748438\\
0.918918918918919	-0.637872204702717\\
0.912912912912913	-0.632928116665062\\
0.906906906906907	-0.628060576386499\\
0.900900900900901	-0.623270644218651\\
0.894894894894895	-0.618559217310264\\
0.888888888888889	-0.613927037674501\\
0.882882882882883	-0.609374700108339\\
0.876876876876877	-0.604902659947999\\
0.870870870870871	-0.6005112406467\\
0.864864864864865	-0.596200641163243\\
0.858858858858859	-0.591970943151824\\
0.852852852852853	-0.587822117945353\\
0.846846846846847	-0.583754033326102\\
0.840840840840841	-0.579766460079021\\
0.834834834834835	-0.575859078324359\\
0.828828828828829	-0.572031483627432\\
0.822822822822823	-0.568283192884448\\
0.816816816816817	-0.564613649984242\\
0.810810810810811	-0.561022231246663\\
0.804804804804805	-0.557508250639081\\
0.798798798798799	-0.554070964773174\\
0.792792792792793	-0.550709577684751\\
0.786786786786787	-0.547423245399882\\
0.780780780780781	-0.544211080291061\\
0.774774774774775	-0.541072155227527\\
0.768768768768769	-0.538005507524195\\
0.762762762762763	-0.535010142693951\\
0.756756756756757	-0.532085038008289\\
0.750750750750751	-0.529229145871478\\
0.744744744744745	-0.526441397013599\\
0.738738738738739	-0.523720703507907\\
0.732732732732733	-0.521065961618103\\
0.726726726726727	-0.518476054481104\\
0.720720720720721	-0.515949854630991\\
0.714714714714715	-0.513486226369807\\
0.708708708708709	-0.511084027990857\\
0.702702702702703	-0.508742113860162\\
0.696696696696697	-0.506459336361665\\
0.690690690690691	-0.504234547711714\\
0.684684684684685	-0.502066601648302\\
0.678678678678679	-0.49995435500045\\
0.672672672672673	-0.497896669143008\\
0.666666666666667	-0.495892411342082\\
0.660660660660661	-0.493940455996148\\
0.654654654654655	-0.492039685777829\\
0.648648648648649	-0.490188992681153\\
0.642642642642643	-0.488387278979027\\
0.636636636636637	-0.48663345809548\\
0.630630630630631	-0.484926455397137\\
0.624624624624625	-0.483265208908222\\
0.618618618618619	-0.481648669953261\\
0.612612612612613	-0.480075803731511\\
0.606606606606607	-0.478545589826998\\
0.600600600600601	-0.477057022657926\\
0.594594594594595	-0.475609111869048\\
0.588588588588589	-0.474200882670465\\
0.582582582582583	-0.472831376126206\\
0.576576576576577	-0.471499649395748\\
0.570570570570571	-0.470204775931563\\
0.564564564564565	-0.468945845635598\\
0.558558558558559	-0.467721964977503\\
0.552552552552553	-0.466532257077248\\
0.546546546546547	-0.465375861754701\\
0.540540540540541	-0.464251935548567\\
0.534534534534535	-0.463159651707006\\
0.528528528528528	-0.462098200152099\\
0.522522522522523	-0.461066787420261\\
0.516516516516517	-0.460064636580541\\
0.510510510510511	-0.45909098713269\\
0.504504504504504	-0.458145094886746\\
0.498498498498498	-0.457226231825798\\
0.492492492492492	-0.456333685953493\\
0.486486486486487	-0.455466761127764\\
0.48048048048048	-0.454624776882161\\
0.474474474474474	-0.453807068236094\\
0.468468468468468	-0.453012985495195\\
0.462462462462462	-0.452241894042965\\
0.456456456456456	-0.451493174124752\\
0.45045045045045	-0.450766220625077\\
0.444444444444444	-0.450060442839236\\
0.438438438438438	-0.449375264240032\\
0.432432432432432	-0.448710122240474\\
0.426426426426426	-0.448064467953156\\
0.42042042042042	-0.447437765947036\\
0.414414414414414	-0.446829494002246\\
0.408408408408408	-0.446239142863532\\
0.402402402402402	-0.445666215992854\\
0.396396396396396	-0.44511022932167\\
0.39039039039039	-0.444570711003346\\
0.384384384384384	-0.444047201166126\\
0.378378378378378	-0.443539251667032\\
0.372372372372372	-0.443046425847063\\
0.366366366366366	-0.442568298287988\\
0.36036036036036	-0.442104454571044\\
0.354354354354354	-0.441654491037774\\
0.348348348348348	-0.441218014553256\\
0.342342342342342	-0.440794642271921\\
0.336336336336336	-0.440384001406147\\
0.33033033033033	-0.439985728997789\\
0.324324324324324	-0.439599471692794\\
0.318318318318318	-0.439224885519019\\
0.312312312312312	-0.438861635667364\\
0.306306306306306	-0.438509396276308\\
0.3003003003003	-0.438167850219928\\
0.294294294294294	-0.437836688899464\\
0.288288288288288	-0.437515612038478\\
0.282282282282282	-0.437204327481649\\
0.276276276276276	-0.436902550997236\\
0.27027027027027	-0.436610006083221\\
0.264264264264264	-0.436326423777152\\
0.258258258258258	-0.436051542469684\\
0.252252252252252	-0.435785107721808\\
0.246246246246246	-0.435526872085776\\
0.24024024024024	-0.435276594929679\\
0.234234234234234	-0.435034042265683\\
0.228228228228228	-0.434798986581875\\
0.222222222222222	-0.434571206677697\\
0.216216216216216	-0.434350487502941\\
0.21021021021021	-0.434136620000245\\
0.204204204204204	-0.433929400951073\\
0.198198198198198	-0.433728632825126\\
0.192192192192192	-0.433534123633123\\
0.186186186186186	-0.433345686782938\\
0.18018018018018	-0.433163140939004\\
0.174174174174174	-0.432986309884967\\
0.168168168168168	-0.432815022389518\\
0.162162162162162	-0.432649112075352\\
0.156156156156156	-0.432488417291209\\
0.15015015015015	-0.432332780986937\\
0.144144144144144	-0.432182050591518\\
0.138138138138138	-0.432036077894014\\
0.132132132132132	-0.43189471892736\\
0.126126126126126	-0.431757833854975\\
0.12012012012012	-0.431625286860104\\
0.114114114114114	-0.431496946037862\\
0.108108108108108	-0.431372683289921\\
0.102102102102102	-0.431252374221769\\
0.0960960960960961	-0.431135898042511\\
0.0900900900900901	-0.431023137467141\\
0.0840840840840841	-0.430913978621244\\
0.0780780780780781	-0.430808310948071\\
0.0720720720720721	-0.43070602711793\\
0.0660660660660661	-0.43060702293986\\
0.0600600600600601	-0.430511197275516\\
0.0540540540540541	-0.430418451955232\\
0.048048048048048	-0.43032869169621\\
0.042042042042042	-0.430241824022782\\
0.036036036036036	-0.430157759188703\\
0.03003003003003	-0.43007641010143\\
0.024024024024024	-0.429997692248337\\
0.018018018018018	-0.429921523624827\\
0.012012012012012	-0.429847824664295\\
0.00600600600600601	-0.429776518169893\\
0	-0.429707529248073\\
}--cycle;
\addplot [color=black, only marks, mark=o, mark options={solid, black}, forget plot]
  table[row sep=crcr]{%
1.13153115619758	-0.83647741955979\\
4.32189755527977	-0.427716025344647\\
};
\end{axis}

==> Figures/acq_n2_v1.tex <==
\begin{axis}[%
width=5.5cm,
height=3cm,
at={(39.75cm,11cm)},
anchor = north east,
scale only axis,
xmin=0,
xmax=6,
xtick={\empty},
ymin=0,
ymax=0.1,
ytick={\empty},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]
\addplot [color=red, line width=1.2pt, forget plot]
  table[row sep=crcr]{%
0	0.017342517425714\\
0.0960960960960957	0.0175661347882903\\
0.174174174174174	0.017853468003648\\
0.24024024024024	0.0182054196113608\\
0.294294294294295	0.0185940052390672\\
0.342342342342342	0.0190366307439218\\
0.39039039039039	0.0195917802822239\\
0.432432432432432	0.0201875841662416\\
0.468468468468468	0.0207927518514159\\
0.504504504504505	0.0214956497612269\\
0.54054054054054	0.0223052269966049\\
0.576576576576577	0.0232281586416727\\
0.612612612612613	0.0242669980070556\\
0.648648648648649	0.0254175777521217\\
0.69069069069069	0.0268811297685092\\
0.804804804804805	0.030981692727023\\
0.828828828828829	0.0316887253183262\\
0.846846846846847	0.0321258177696464\\
0.864864864864865	0.0324560415711197\\
0.882882882882883	0.0326513084864279\\
0.894894894894895	0.0326909824864083\\
0.906906906906907	0.0326463064661056\\
0.918918918918919	0.0325062081433849\\
0.930930930930931	0.0322588896094453\\
0.942942942942943	0.031891855742824\\
0.954954954954955	0.0313919602503834\\
0.966966966966967	0.0307454727829226\\
0.978978978978979	0.0299381711084461\\
0.990990990990991	0.0289554629477449\\
1.003003003003	0.0277825428022656\\
1.01501501501502	0.0264045899555096\\
1.02102102102102	0.0256341501394823\\
1.02702702702703	0.0248070148350799\\
1.03303303303303	0.023921446160176\\
1.03903903903904	0.0229757621203506\\
1.04504504504505	0.0219683498916883\\
1.05105105105105	0.0208976804201635\\
1.05705705705706	0.0197623244486103\\
1.06306306306306	0.0185609700925875\\
1.06906906906907	0.017292442097979\\
1.07507507507508	0.0159557229261544\\
1.08108108108108	0.014549975827336\\
1.08708708708709	0.0130745700798132\\
1.09309309309309	0.0115291085926996\\
1.0990990990991	0.00991345809492028\\
1.10510510510511	0.00822778216848175\\
1.11111111111111	0.00647257745218255\\
1.11711711711712	0.0046487135635962\\
1.12312312312312	0.00275747872888754\\
1.12912912912913	0.00080066614161467\\
1.13513513513514	0.00119740842854021\\
1.14114114114114	0.00314127657663299\\
1.14714714714715	0.00501915365800709\\
1.15315315315315	0.00682936590333938\\
1.15915915915916	0.00857071302412571\\
1.16516516516517	0.0102424034545248\\
1.17117117117117	0.0118440102729336\\
1.17717717717718	0.0133754320953106\\
1.18318318318318	0.0148368575381115\\
1.18918918918919	0.0162287327773054\\
1.1951951951952	0.0175517318962433\\
1.2012012012012	0.0188067297728249\\
1.20720720720721	0.0199947772888596\\
1.21321321321321	0.0211170786682198\\
1.21921921921922	0.0221749707697771\\
1.22522522522523	0.0231699041775908\\
1.23123123123123	0.0241034259452588\\
1.23723723723724	0.0249771638640048\\
1.24324324324324	0.0257928121353537\\
1.24924924924925	0.026552118339298\\
1.26126126126126	0.0279088918420021\\
1.27327327327327	0.0290621097101988\\
1.28528528528529	0.0300266013683537\\
1.2972972972973	0.0308171591603976\\
1.30930930930931	0.0314483447738665\\
1.32132132132132	0.0319343361765849\\
1.33333333333333	0.0322888089762552\\
1.34534534534535	0.0325248469508255\\
1.35735735735736	0.0326548772115105\\
1.36936936936937	0.0326906260726485\\
1.38138138138138	0.0326430922301446\\
1.3993993993994	0.0324378744086733\\
1.41741741741742	0.0320996861643756\\
1.43543543543544	0.0316563758748289\\
1.45945945945946	0.030943379153876\\
1.48948948948949	0.0299230231567229\\
1.54354354354354	0.0279368263802233\\
1.5975975975976	0.0259891429466945\\
1.63363363363363	0.0247905658577965\\
1.66966966966967	0.0236985287952072\\
1.70570570570571	0.0227214807120717\\
1.74174174174174	0.0218596280615504\\
1.77777777777778	0.0211079472875433\\
1.81381381381381	0.020458360491256\\
1.85585585585586	0.0198166839709764\\
1.8978978978979	0.0192848139624813\\
1.94594594594595	0.0187913845145351\\
2	0.0183566742484205\\
2.06006006006006	0.017992275177086\\
2.12612612612613	0.0177012686641502\\
2.2042042042042	0.0174647334118747\\
2.3003003003003	0.0172811729244264\\
2.43243243243243	0.0171437393005913\\
2.63663663663664	0.0170517615395767\\
3.06306306306306	0.0168787602403109\\
3.1951951951952	0.0167061425659263\\
3.29129129129129	0.0164761215499487\\
3.36936936936937	0.0161812009878757\\
3.43543543543544	0.0158203812573037\\
3.48948948948949	0.0154223550631913\\
3.53753753753754	0.0149693331989251\\
3.57957957957958	0.014479619503537\\
3.62162162162162	0.0138869022748676\\
3.65765765765766	0.0132847391259112\\
3.69369369369369	0.0125851506606667\\
3.72972972972973	0.0117791135714951\\
3.76576576576577	0.0108597900637726\\
3.8018018018018	0.00982429290279452\\
3.83783783783784	0.008676105837786\\
3.87987987987988	0.00721216084073983\\
3.93993993993994	0.00498043900061074\\
3.98798798798799	0.00322687805781818\\
4.01801801801802	0.00223602641346066\\
4.04204204204204	0.00154564105219457\\
4.06606606606607	0.000974487416553593\\
4.08408408408408	0.000636043577721068\\
4.1021021021021	0.000378545413407316\\
4.12612612612613	0.000155381660018605\\
4.15015015015015	4.54673120477977e-05\\
4.18618618618619	2.25126257102914e-06\\
4.45645645645646	1.97110128308253e-06\\
4.4984984984985	6.03965364280867e-05\\
4.52252252252252	0.000190234101720144\\
4.54654654654655	0.000439981173084192\\
4.56456456456456	0.000719279540432716\\
4.58858858858859	0.00121646391468744\\
4.61261261261261	0.00184440035018518\\
4.63663663663664	0.00258039319367498\\
4.66666666666667	0.00361041297717701\\
4.71471471471471	0.00538819915662359\\
4.77477477477477	0.00760130340203613\\
4.81681681681682	0.00903341186491691\\
4.85285285285285	0.0101484999093335\\
4.88888888888889	0.0111490029037542\\
4.92492492492492	0.0120336541166823\\
4.96096096096096	0.0128067536984844\\
4.996996996997	0.013475956284041\\
5.03903903903904	0.014137989476672\\
5.08108108108108	0.0146874623208086\\
5.12912912912913	0.0151978168906597\\
5.17717717717718	0.0156035674560178\\
5.23123123123123	0.0159588747380717\\
5.2972972972973	0.0162798736037786\\
5.37537537537538	0.0165412664709583\\
5.47147147147147	0.0167441703035989\\
5.59159159159159	0.01688535145919\\
5.77177177177177	0.0169784030034075\\
6	0.0170154612047977\\
};
\end{axis}

==> highlights.tex <==
\item A system identification method using machine learning techniques to avoid overfitting
\item Bayesian optimization for hyperparameter tuning, selecting model inputs and structure
\item Excellent performance for the closed-loop identification of a MSW grate incinerator
\item Modelling of fuel disturbance effects using flue gas measurements
\item Complete MSW grate incineration models in continuous time are given


